Closed categories

We are checking the closed categories beginning with the category of sets and ending with the category of categories. The novelty is a generalizing the notion of adjoint functors to the joint pair of functors in the category of directed graphs. We have described for what condition we get a bijective name mapping for graphs transports. Graphs aren't instances of categories, however we believe that new notion of functors joint pair will become important also for the categorical studies. As an example of future applications we introduce the notion of relator to some tensor product.

==> closed.tex <==
%2022.05.08. Pradójau traukõ clattice/closed.tex
%2022.08.30. Taisiau
%2022.09.10. Gal jau galutinis, dar truputõ
\Skyr Closed categories.  Closed categories..
 The  scalar space
$V=[0;\infty]$  was the first example of ^{closed monoidal =category}.
It was ^{values  =space} for metric spaces.
 Its objects were  called ^{=values} and arrows $r\rightarrow s$ were
 inequality  between values
$r\dgl s$.

The monoidal category has  a tensor product $r\otimes s$ defined with
some  ^{=bifunctor}. For arbitrary ^{binary =word of objects} we define  the
tensor product of these objects ^{=uniquely up to unique
canonical isomorphism}.
The monoidal category is closed if its tensor product defines
functor $r\otimes s$ having coadjoint functor $t^s=\exp_t s$.
It will be called an  ^{ exponential =functor}.
Otherwise for exponential functor $t^s$ tensor product $r\otimes s$ will
be an adjoint functor. We shall say that both functors provide
a ^{joint =pair of functors}, The first functor is adjoint to the second, and the
second is coadjoint to the first.
For ^{truly =joint pair of functors} we have  ^{natural =bijection}
between arrows sets
$$V(r\otimes s; t)=\rightarrow V(r; t^s)\tsk$$
For an arrow $f: r\otimes s\rightarrow t$ this bijection
appoints its ^{=name}
$\lceil f\rceil: x\rightarrow t^S$.
The inverse bijection  will be called a ^{=cobijection } of taken joint pair
of functors
$$V(r;t^s)=\rightarrow V(r\otimes s;t)\tsk$$
It for the arrow $g: x\rightarrow t^s$ appoints its ^{=realization }
$\lfloor g \rfloor : r\times s\rightarrow t$.

We extend the notion of joint pair of functors for more general case.
The ^{=joint pair of functors} from category $X$ to category $Y$
will be arbitrary pair of functors
$$\lan F, G\ran : X\rightleftarrows Y\tsk$$
One $F:X\doublerightarrow Y$ is called an ^{adjoint =functor}, another
$G: Y\doublerightarrow X$ is called a ^{coadjoint =functor}.
A ^{=unit
transform} $i:\Identity_X\rightarrow FG$ is defined by collection
of arrows $i_x: x\rightarrow x^{FG}$ for every point in the source category
$x\in X$. Sometimes such arrows haven't any
property needed in source category $X$, so unit transform for joint pair
of functors is only auxiliary.  The existing unit transform
defines  a name mapping between arrows sets
$$ Y(x^F;y)\rightarrow X(x;y^G)\tsk$$
For an arrow $f\in Y(x^F;y)$ it appoints the composition  of unit arrow with
image of
taken arrow for the adjoint  functor
$i_x\circ f^G\in X(x;y^G)$.
For a natural unit transform we get
the natural name mappings  with respect to
arrows in each category $u\in X(x';x)$ and $v\in Y(y;y')$.
$$\matrix { Y((x')^F; y') &\rightarrow & X(x'; (y')^G)\cr
 \mapupk (u^F)^*\times v_* & & \mapupd u^*\times (v^G)_* \cr
 Y(x^F; y) & \rightarrow & Y(x;y^G)\cr} $$
\vskip \tarpas
It can be expressed as commuting diagrams in the category $X$
$$\matrix { x'& \mapright i_{x'} & (x')^{FG} & \mapright (f')^G  & (y')^G \cr
          \mapdownk u &  &\mapdownk u^{FG} & & \mapupd v^G \cr
          x& \maprightap i_x & x^{FG} & \maprightap f^G & y^G \cr }$$
\vskip\tarpas
A ^{counit =transform} $e: GF\rightarrow \Identity Y $
is defined by collection of arrows $e_y: y^{GF}\rightarrow y $
for every point in the target category $y\in Y$.  The counit transform for joint
pair of functors is also only auxiliary.  The existing counit transform
defines a ^{=realization mapping}  between former arrows sets in opposite
direction
$$X(x;y^G) \rightarrow Y(x^F;y)\tsk$$
For an arrow $g\in X(x;y^G)$ it appoints the composition of image
for the coadjoint functor of taken arrow with counit arrow
$g^F\circ e_y \in Y(x^F;y) $.
For a natural counit transform we get the natural realization mapping according
to the arrows in each  category $u\in X(x';x) $ and $v\in Y(y;y')$
$$\matrix { X(x'; (g')^G) & \rightarrow & Y((x')^F; y') \cr
     \mapupk  u^*\times (v^G)_*  &    & \mapupd (u^F)^*\times v_*  \cr
     X(x;g^G) & \rightarrow  &  Y(x^F;y) \cr } $$
\vskip\tarpas
It can be expressed  as commuting diagrams in category $Y$
$$\matrix { (x')^F & \mapright (g')^F & (y') ^{GF} & \mapright e_{y'}  & y' \cr
         \mapdownk u^F  &  & \mapdownk (v)^{GF}  &  & \mapupd v  \cr
         x^F & \maprightap g^F  & y^{GF} & \maprightap e_y & y \cr } $$
\vskip \tarpas

For  ^{truly =joint pair of functors}
we demand that realization mapping would be inverse to the name mapping, i. e.
both mappings would be bijections. We shall say that a realization mapping
^{=reverses} the name mapping, and a name mapping reverses the
realization mapping.

Taking an arrow $f=1_{x^F}$ we construct its name's realization.
It coincides with arrows composition
$$(i_x)^F\circ e_{(x^F)}: x^F\rightarrow x^F \tsk$$
So if the realization mapping ^{=reverses} name mapping  we get the ^{first
triangular =equality}  for unit and counit transforms
$$i\times F\circ F\times e = \Identity_F\tsk$$

Otherwise, having the first triangular equality the realization of name maps
the same arrow $f\in Y(x^F;y)$ exactly when we have commuting quadrat
begun with an arrow $(i_x)^ F: x^F\rightarrow x^{FGF} $
for the unit transform ended with the adjoint functor
$$\matrix {x^F & \mapright i\times F & x^{FGF} & \mapright f^{GF}  & y^{GF} \cr
               &               & \mapdownd F\times e &  & \mapdownd e \cr
               &                    &x^F & \maprightap  f & y \cr} $$
\vskip\tarpas
This can be proved by completing the first triangular diagram
with the unit arrow of identity  transform $\Identity_F:F\rightarrow F$
$$\matrix {x^F & \mapright i\times F & x^{FGF} & \mapright f^{GF}  & y^{GF} \cr
               &\searrow               & \mapdownd F\times e &  & \mapdownd e \cr
               &                    &x^F & \maprightap  f & y \cr} $$
\vskip\tarpas

Taking an arrow $g=1_{y^G}$ we construct its realization's name .
It coincides with arrows composition
$$(i_{(y^G)}\circ (e_y )^G: y^G\rightarrow y^G \tsk$$
So if  the name  mapping ^{=reverses}  realization mapping we get the ^{second
triangular =equality}  for unit and counit transforms
$$(G\times i)\circ (e\times G)= 1_G \tsk$$

Otherwise,  having the ^{second triangular =equality} the name of realization
maps the same arrow $g\in  X(x;y^G)$  exactly when  we have
commuting quadrat ended with an arrow $ (e_y)^G: y^{GFG}\rightarrow x^G$
for the counit transform ended with the coadjoint functor
$$ \matrix { y^G & \mapleft  e\times G & y^{GFG} & \mapleft  g^{FG} & x^{FG} \cr
                 &       & \mapupd G\times i &   & \mapupd i  \cr
                 &           & y^G &\mapleftap  g & x \cr} $$
\vskip\tarpas
This can be proved by completing the second triangular diagram
with the unit arrow of identity transform $\Identity_G: G\rightarrow G$
$$ \matrix { y^G & \mapleft  e\times G & y^{GFG} & \mapleft  g^{FG} & x^{FG} \cr
                 &\nwarrow        & \mapupd G\times i &   & \mapupd i  \cr
                 &           & y^G &\mapleftap  g & x \cr} $$
\vskip\tarpas

For natural unit and counit transforms the first and second triangular
equalities provides that the name mapping and the realization mapping are
inverse each to other natural bijections
$$Y(x^F;y) =\rightarrow X(x;y^G) \tsk$$

In monoidal category $\VV$ else we have a ^{final =object} $*\in \VV$, i. e.
for every object $r\in V$ we always have exactly one arrow $!:r\rightarrow *$.
We demand that final object $* \in \VV$ would be also the ^{ =unit
for tensor product},
i. e. we should have canonical isomorphisms
$$*\otimes r= r=r\otimes *\tsk$$

We shall look for^{ exponential  =functor} in various categories.
At first we shall probe  to define the exponential functor
in the category of all sets $\SET$  or in the category of
^{small =sets} $\Set$.
Then the most familiar will be the case of the category $\CAT$ of
all possible categories. The ^{arrows =set} $\CAT(X;Y)$  will be
compounded of functors $f: X\doublerightarrow Y$
between categories $X$ and  $Y $,  The exponential functor
will be coadjoint for the ^{Carte tensor =product}. It  for a category $X$
appoints the category $X^A$ with
 arrows sets $X^A(f;g)$ compounded of all natural transforms
 $\phi: f\rightarrow g$ between functors $f,g: A\doublerightarrow X$.

In next part of this work the construction of such arrows sets will be
rewritten for the
category $\Cat_{\Set}$ of $\Set$-enriched categories with values
category $\Set$ of small sets. It will be a sample for a  construction
of exponential functor in the category $\Cat_{\VV}$ of $\VV$-enriched
categories for arbitrary values category $\VV$. So we acquire the construction
of exponential functor also in the category of metric spaces
$\Cat_{[0,\infty]}$.
Finally we shall construct exponential functor in the category $\Cat_{\VV}$
with another tensor product in  values category $\VV$
which will be called a ^{=relator} to the original tensor product of
closed  monoidal category $\VV$. Then we provide the proving of Yoneda lemma
for $\Set$-enriched categories.
The exponential functor is needed
for the $\VV$-enriched category $X$ to  define  the second dual space
$\hat X =\VV^{X^\op} $
with Yoneda imbedding $X\subset \hat X$.
\vskip\tarpas


We could work with the category of all sets $\SET$.  We shall define exponential functor
in such tremendous category.
The objects of category $\SET$ will be arbitrary  sets $X$ as entity
of points $x\in X$. They will be called  ^{=members of taken set}.
The arrows between two sets will be arbitrary  appointment
$f: X\rightarrow Y$. It for each member in the source set $x\in X$
appoints the member in the target set $f(x)\in Y$.
For appointments $f: X\rightarrow Y$ and $g: Y\rightarrow Z$
we have usual composition $f\circ g: X\rightarrow Z$ with
$$f\circ g(x)= g(f(x))\kbl$$
and we can choose identity appointments $\Identity_X: X\rightarrow X$
with  $\Identity_X(x)=x $ for each point $x\in X$
as unit arrows for such composition
$$\Identity_X\circ f= f=f\circ \Identity_Y \tsk$$

In the category $\SET$ we shall define  the tensor product of two sets
$X\times Y$. It will be a set of all pairs
$$X\times Y= \lbrace \lan x,y\ran: x\in X, y\in Y\rbrace$$
We take two appointments
$p_1: X\times Y\rightarrow X$ and
$p_2:X\times Y\rightarrow Y$
$$p_1(\lan x, y\ran)= x\kbl p_2(\lan x,y\ran) =y\tsk$$
as projections of taken tensor product.

It will provide one ^{possible =realization of the Carte product} in
the category $\SET$, i. e. we can check the ^{universal =property
of such product}. For arbitrary two  appointments
$f:Z\rightarrow X$ and $g:Z\rightarrow Y$ we have exactly one
appointment to the product
set $h:Z\rightarrow X\times Y$
with projections equal to taken  appointments
$$h\circ p_1= f\kbl h\circ p_2= g\tsk$$
It can be  taken
 $$h(z)= \lan f(z),g(z)\ran \in X\times Y\kbl $$
 and if we have some  appointment
$h': Z\rightarrow X\times Y$ with taken projections,
then for the point $z\in Z$
appointed  pair $h'(z)= \lan x,y\ran \in X\times Y$
will have  the same projections
$$ x= h'\circ p_1 (z)= f(z)\kbl y= h'\circ p_2 (z)=g(z)\kbl$$
therefore we have equality of appointed pairs
$\lan x,y\ran = \lan f(z),g(z)\ran $ and  equality of both appointments
$$h'= h\tsk$$

Using universal property of the Carte product we get   unique
isomorphisms
$$S_{X,Y,Z} : X\times (Y\times Z)\rightarrow (X\times Y)\times Z\tsk$$
These isomorphisms are natural for possible appointments
$$f: X\rightarrow X'\kbl g: Y\rightarrow Y'\kbl h: Z\rightarrow Z'\tsk$$

They admit the  ^{pentagon =diagram}, so we can get coherence property
from \baf MacLane 1971* part VII. Monoids to get tensor product
for arbitrary binary word
of   sets ^{=uniquely up to unique canonical isomorphism}.
In our  case the ^{canonical =isomorphisms} are chosen
next appointments  and their  inverse together with all possible
compositions of various tensor products. First we take
identity  appointment of any taken set $1_X:X\rightarrow X$,
secondly we take former isomorphism of associativity
$S_{X,Y,Z}$.

Any onepoint set $*=\lbrace o\rbrace$ provides final object in the category
$\Set$. It becomes unit for the tensor product with
chosen canonical isomorphisms
$$R_X: X\times *\rightarrow X $$
which for a couple $\lan x,o\ran\in X\times *$ appoints the point $x\in X$,
and $$L_X: *\times X\rightarrow X$$
which for a couple $\lan o,x\ran \in *\times X$ appoints the point $x\in X$.

Every  onepoint set $*=\lbrace o'\rbrace$  correspondingly will
provide another  ^{possible =realization  of  the final object}
in the category $\Set$. It can be taken as another unit
for taken product  with
another natural isomorphisms for the projections
$$R_X: X\times *\rightarrow X\kbl L_X: *\times X\rightarrow X\kbl$$
These projections are natural transforms.
It rests to check that such projections are isomorphisms.

For the projection $R_X: X\times *\rightarrow X$ we take an appointment
to the product $\theta:X\rightarrow X\times *$ defined with
 the pair of appointments
 $1_X: X\rightarrow X$ and unique  appointment
  to the final object
$!: X\rightarrow *$, i. e. we have composition equal to the identic
appointment
$$\theta\circ R_X= 1_X\tsk$$
Otherwise the composition $R_X\circ \theta: X\times *\rightarrow X\times *$
is unanimously defined by the projections. One projection is
$$(R_X\circ \theta)\circ R_X = R_X\circ (\theta\circ R_X)= R_X\kbl$$
and another coincides with unique arrow to the final object
$$(R_X\circ \theta)\circ != ! \tsk$$
Therefore we get another equality
$$R_X\circ \theta= 1_X\times 1_*= 1_{X\times *} \tsk$$

These projections admit the ^{triangular cancellation =diagrams}.
Such diagrams
were  drown in \baf G. Valiukevi\v cius 1992* p. 144.

And finally we get equal projections $R_*= L_* $, as the product of
onepoint set is contained in the diagonal of product
$$\trik = *\times * \tsk$$

So we have got a tensor product for monoidal category
of \baf B\' enabou 1963*. We shall call it  a ^{Carte tensor =product}.
Usually  we understand  the Carte product  more freely as a final object in the
category of cones over ^{discrete =diagrams of factors}.  In
\baf G. Valiukevi\v cius 2009* p. 13 we have discussed ^{abstract =objects }
investigated in the theory of categories. Such theory was announced
by one of its exploiter Norman Steenrod
as ^{abstract =nonsense}.
The Carte product is an example of such abstract objects.
Otherwise the topology in general sense
by G. Valiukevi\v cius deals with mappings of concrete objects. Functors
 will be examples of continuous mappings
in some topological spaces
and tensor products in category is defined as a family of
concrete objects with unique ^{canonical =isomorphisms} between different
realizations  of some finite tensor product.

 The importance of abstract objects has become evident in the science
of program writing for any computer. The programs are written in abstract
way, without trouble about concrete processes fulfilling such calculations.

We wish that the category of all sets $\SET$  would be  a
^{closed monoidal =category}.

The Carte tensor product of two sets $X\times Y$
defines bifunctor
$$\SET\times \SET \doublerightarrow \SET\tsk$$
For a  pair of  sets $\lan X,Y\ran $ we appoint the new set $X\times Y$,
and for  a pair of appointments $f: X\rightarrow X'$ and $g: Y\rightarrow Y'$
we get the product of appointments
$$f\times g: X\times Y\rightarrow X'\times Y'$$
which for a pair of points $\lan x,y\ran\in X\times Y$ appoints
the pair of appointed points $\lan f(x),g(y)\ran\in X'\times Y'$.

Additionally we have maintenance of arrows composition
$$(f\times g)\circ (f'\times g')= (f\circ  f')\times ( g\circ g')\kbl$$
and maintenance of unit arrows
$$\Identity_X\times \Identity_Y= \Identity_{X\times Y} \tsk$$

The chosen onepoint set $*=\lbrace o\rbrace$ with correspondent
isomorphic projections
$$R_X: X\times *\rightarrow X\kbl L_X: *\times X\rightarrow X$$
becomes a ^{=neutral set} for taken Carte tensor product.

For arbitrary ^{=assistant set} $T$ the Carte tensor product
defines a functor denoted $X\times T$
$$\SET\doublerightarrow \SET$$
which for arbitrary set $X$ appoints the Carte tensor product $X\times T$
and for arbitrary appointment $f: X\rightarrow X'$ appoints another
appointment provided as Carte product of appointments
$f\times \Identity_T: X\times T\rightarrow X'\times T$.

Now we shall construct
a coadjoint exponential functor $Y^T$.
For arbitrary  set $Y$ we appoint the ^{functional =space}
$Y^T$ compounded of
all possible appointments over assistant set
$\phi: T\rightarrow Y$.

For an appointment $f:Y\rightarrow Y'$  this functor appoints
the appointment  of functional spaces
$f^T: Y^T\rightarrow (Y')^T$, which for an
appointment $\phi\in Y^T$  provides
the composed appointment $\phi\circ f\in (Y')^T$.
We shall call such composition as ^{=changing of target space} $Y$.

We shall check that we have got a ^{truly joint =pair of functors}
$$\lan F,G\ran :\SET \rightleftarrows \SET $$
defined with Carte tensor product $X^F= X\times T$ and functional space
$Y^G= Y^T$.

The ^{=unit transform of  joint pair} $i: \Identity_{\SET}\rightarrow FG$
will be  defined with collection of ^{sections =appointments}
$$\lambda_X: X\rightarrow (X\times T)^T$$
which for a point $x$ appoints the ^{=section}
$\lambda_X (x)\in (X\times T)^T$, i. e. a graph of constant
appointment $\lambda_X(x)_t=\lan x,t\ran$.

We get  a ^{natural =transform} of functors
as  for arbitrary appointment  $f: X\rightarrow X'$
we have commuting diagram:
\vskip\tarpas
$$\matrix{ \hskip 8 pt  X & \mapright f  & X' \hskip 10 pt\cr
   \mapdownk_{\lambda_X} & & \mapdownd_{\lambda_{X'} } \cr
  ( X\times T)^T &\maprightap {(f\times 1)}^T & (X'\times T)^T \cr }$$
\vskip\tarpas
Indeed. The section $\lambda_X(x)\in (X\times T)^T$
which for the argument $t\in T$
appoints a couple $\lan x,t\ran\in X\times T$ now will be transformed to
a new section which for the argument $t\in T$ will appoint a couple
$\lan f(x), t\ran \in X'\times T$,
therefore this new section is get by composition $f\circ \lambda_{X'}$.

The ^{=counit transform of joint pair} $e: GF\rightarrow \Identity_{\SET} $
will be defined with collection of  ^{=evaluation  appointments}
$$\ev_Y: Y^T\times T \rightarrow Y$$
 which for an appointment $f\in Y^T$ and a
point $t\in T$ appoints the value of taken appointment over taken point
$f(t)\in Y$.
These arrows define a natural transform of functors
 as for arbitrary  mapping $
g: Y\rightarrow Y'$ we get commuting diagram
\vskip\tarpas
$$\matrix{ (Y^T)\times T  & \mapright {g^T \times 1} & (Y')^T\times T \cr
        \mapdownk {\ev_Y } & & \mapdownd \ev_{Y'} \cr
        \hskip 15 pt Y & \maprightap g & Y'\hskip 15 pt  \cr } $$
\vskip \tarpas
Indeed. For a mapping $g: Y\rightarrow Y'$  the composition of functors
$GF$
appoints the  mapping  $Y^T\times T\rightarrow (Y')^T\times T$
which for an appointment $\phi\in Y^T$ and a point  $t\in T$ provides
the composed function $\phi \circ g\in (Y')^T$ and the
same argument $t\in T$,
therefore the new evaluation $\ev_{Y'}$  will provide the value
$g(\phi(t))$ which
coincides with value appointed by composition  $\ev_X\circ g$.


For the ^{truly =joint pair of functors}
we additionally must check both ^{triangular =equalities}.
At first I shall explain  the notation for ^{horizontal =composition
of natural transforms}
$s; F\rightarrow G$ and $t: K\rightarrow L$
between functors $F,G: A\doublerightarrow B$ and $K,L: B\doublerightarrow C$
with $s\times t: FK\rightarrow GL$ defined with composition of
arrows
$$s^K_a:a^{FG}\rightarrow a^{GK}\kbl t_{a^G}: a^{GK}\rightarrow a^{GL}\kbl$$
or another equal composition
$$t_{a^F}: a^{FK}\rightarrow a^{FL}\kbl s^L_a: a^{FL}\rightarrow a^{GL}\tsk$$
So we have an equality
$$s_a^K\circ t_{a^G} = t_{a^F}\circ s^L_a \tsk$$

For a functor $F: A\doublerightarrow B$ we
take  the identity transform
$\Identity_F: F\rightarrow F$ and define the horizontal composition
$$F\times t= \Identity_F\times t$$
which is defined with  collection of arrows
$t_{a^F}:a^{FK}\rightarrow a^{FL}$.

And for a functor $K$ we can use the horizontal composition
$$s\times K= s\times \Identity_K\kbl$$
it is defined with  new arrows $s_a^K: a^{FK}\rightarrow a^{GK}$,
More about horizontal composition can be seen in \baf G. Valiukevi\v cius
1992* p. 98.

The first triangular equality is for the unit transform
 ended with the  adjoint
functor
and composed with the counit transform begun with the same adjoint functor
$$i\times F\circ F\times e = 1_F\tsk$$
For a set  $X$ we take the Carte tensor product $X\times T$ and we must check
that we shall get the composition of two natural mappings equal to
the identity mapping. The first natural transform $i\times T$ for a
couple $\lan x,t\ran \in X\times T$ will appoint the couple of
section $\lambda_X(x)\in (X\times T)^T$ and the same point $t\in T$
$$\lan \lambda_X(x),t\ran \in (X\times T)^{T}\times T \tsk$$

The second transform  is an evaluation for the space
$X\times T$.
It for a section $\lambda_X(x)$ appoints its value over the point
$t\in T$,
therefore we get the same value $\lambda_X(x)_t= \lan x,t\ran \in X\times T$.

The second triangular equality is defined for the unit transform begun
with the coadjoint functor
and composed with the counit transform  ended with the same coadjoint functor
$$G\times i\circ e\times G=1_G\tsk$$
This composition must be the identity transform  over functional space $Y^T$
which is appointed by coadjoint functor $G$ for taken set $Y$.

The unit transform is defined with sections appointments
$$\lambda_{Y^T}: Y^T\rightarrow (Y^T\times T)^T\tsk$$
They  for an appointment
$\phi\in X^T$ will appoint the  section
$\lambda_{Y^T}(\phi)$ with values
$$\lambda_{Y^T}(\phi)_t= \lan \phi,t\ran \tsk$$
Such section   will be a point from
functional space appointed by coadjoint functor $G$
for the space $Y^T\times T$
$$\lambda_{Y^T}(\phi)\in (Y^T\times T)^T\kbl $$
therefore the counit appointment  first
will be applied as evaluation
$$\ev_Y:Y^T\times T\rightarrow Y$$
and then will be changed
by coadjoint functor, i. e. we  transform  the  function
$\psi\in Y^T$ by changing target space with   evaluation arrow.
For taken function it will be appointed composed function
$\psi\circ \ev_Y$.

The  section
$\lambda_{Y^T} (\phi): T\rightarrow  Y^T \times T$  will be  appointed
to appointment  which for the point $t\in T$ appoints evaluation of
taken appointment over taken  point $t$. Therefore we get the
same appointment $\phi$.

So we have checked that category $\SET$ is a monoidal closed category.
\vskip\tarpas


In some cases we need to work with ^{small =sets}
by means of \baf S. MacLane 1971* part 1 \S6. It means the  members from some
^{=universe} $U$. This was a problem of logic to say what is a set
of all sets
which aren't members of itself. Therefore it was proposed to work only
with members of some large set $U$, which is called a universe.
It was demanded

that every member $x\in y$ of any small set $y\in U$ would be again a small
set $x\in U$,

the product of small sets $u\in U$, $v\in U$
remains small set  $u\times v\in U$,

for small set $u\in U$ the union  of members $\Cup u$ remains small set

and  the set of all subsets $2^U$  remains a small set,

the set of all finite ordinals $\VN$ is a small set $\VN\in U$,

for arbitrary function $f: X\rightarrow Y$ the image of small
set $u\in U$ remains  small set $f(u)\in U$.

Also we use the principle  of comprehension that the members of small set
with some logical property  $\phi$
$$\lbrace x: x\in u, \phi(x)=\true \rbrace $$
remains small set.

The small sets were
applied by \baf N. Bourbaki Th\'eorie des ensembles 1957* to construct
a  ^{universal =arrow}. Later we shall use small topological
space to construct
strongest Hausdorff
simplification.

We shall work with  a category of small sets. It again will be a closed
monoidal category with Carte tensor product and coadjoint
exponential functor.

The objects of category $\Set$ will be arbitrary small sets $X$,
and the arrows will be arbitrary mappings between small sets $f: X\rightarrow Y$.
It can be identify with graphics as partial set $f\subset X\times Y$, therefore
the whole arrows set $\Set (X;Y) \subset 2^{X\times Y}$ remains small set.

Obviously we have an imbedding of categories $\Set\subset \SET$.


The Carte tensor product of small sets
$$X\times Y= \lbrace \lan x,y\ran: x\in X,y\in Y\rbrace $$
remains a small set.  So we have got a tensor product in the category $\Set$
with the same neutral onepoint set $*= \lbrace o\rbrace$.

We shall check that the category of small sets $\Set$
again is  a
^{closed monoidal =category}, i. e. for the functor provided
with Carte tensor product $X\otimes T$ we get
a coadjoint exponential functor $Y^T$.

For small  assistant set $T$ and another small set $Y$
 we appoint the ^{functional =space}
$Y^T$ compounded of
all possible mappings $\phi: T\rightarrow Y$, i. e. it is contained
in the small set $\two^{T\times Y}$.

For the mapping $g:Y\rightarrow Y'$  this functor appoints a
mapping of functional spaces provided by changing target space
$g^T: Y^T\rightarrow (Y')^T$, which for a function $\phi\in Y^T$  provides
the composed
function $\phi\circ g\in (Y')^T$.

In imbedded smaller category $\Set\subset \SET$ we get again
a truly joint pair of  induced functors
$$\lan F_0,G_0\ran:\Set\rightleftarrows \Set\kbl$$

as  we have the unit transform
$i: \Identity_{\Set}\rightarrow  F_0G_0$ and the counit  transform
$e: G_0F_0\rightarrow \Identity_{\Set}$
defined with arrows from smaller category $\Set$,  i. e.
these arrows are mappings between small sets
$$\lambda_X: X\rightarrow (X\times T)^T\kbl
 \ev_Y: Y\times T\rightarrow Y\tsk$$
\vskip\tarpas

Next we shall construct  an exponential functor
in the category  $\CAT$ of all categories. But first we shall stop a little
with a category o all directed graphs $\GRPH$.

The graph is defined
as a set of edges $X$ between vertexes from set $X_0$.
We have two projections
 $p_1,p_2: X\rightarrow X_0$. One $p_1$ is for the source of edges, and
 another $p_2$ for the target of edges.
Between arbitrary two vertexes $a,b\in X$ we define  an edges set
as the inverse image of both projections
$$X(a;b)= (p_1\times p_2)\inv (\lan a,b\ran)\uparrow
\lan a,b\ran\in X_0\times X_0\tsk$$

 The transport of graphs
 $f: X\doublerightarrow Y $ will be defined by a mapping of edges
 $f: X\rightarrow Y$ and a mapping for vertexes $f_0: X_0\rightarrow Y_0$.
These two mappings must commute with source and target projections
$$\matrix { X&\mapright f & Y\cr
\mapdownk p_1 & &\mapdownd p_1 \cr
 X_0 & \maprightap f_0 & Y_0 \cr}
\hskip 30 pt
\matrix{
X&\mapright f & Y\cr
\mapdownk p_2 & &\mapdownd p_2 \cr
 X_0 & \maprightap f_0 & Y_0 \cr} $$

A transport of graphs can be  defined with collection of mappings over
edges sets
$$f_{a,b}: X(a;b) \rightarrow X(f_0(a);f_0(t))\tsk$$

If the projections of arrow's source or target would be understood as
an instance of convergence in the set $X_0$ of vertexes for the sequences
defined with one edge, then transport of mappings can be viewed as
continuous mappings $f: X_0\rightarrow Y_0$
for such convergences in the spaces of vertexes.

Arbitrary category $X$ is an example of graph. The edges will be called
as arrows,
and the vertexes will be called as points. Additionally we define composition
of arrows. It is functional mapping defined over the
^{=pullback of projections}
$$X\times _{X_0} X\rightarrow  X\tsk$$
Such mapping can be  defined with  collection of mappings over arrows sets
$$X_{a,b,c}: X(a;b)\times X(b;c)\rightarrow  X(a;c)\tsk$$
We can  denote this operation by its image set
$$X(a;b)\times X(b;c)\rightarrow X(a;b)\circ X(b;c)\subset X(a;c)\tsk$$

We demand associativity for mappings of arrows composition. It can be
expressed as equalities
$$X(a;b)\circ (X(b;c)\circ X(c;d))= (X(a;b)\circ X(b;c))\circ X(c;d)\tsk$$

For the ^{true =category} we also need an appointment of unit arrows
$$1_a\in X(a,a)\tsk$$
We demand that for an arrow $u\in X(a;b)$ the appointed arrows would  be
neutral for ^{=composition before arrow}
$$1_a\circ u= u \kbl$$
and  ^{=composition after arrow}
$$u\circ 1_b= u  \tsk$$

The categories without unit arrows can be called as ^{=semicategories},
together
with ^{=semimonoids} or ^{=semigroups}. The structure of such algebraic objects
would become much more delicate.

In \baf G. Valiukevi\v cius 2009* I proposed to call algebraic operation of
composition as a convergence for finite sequences of two members, and
the appointment of unit arrows as a convergence for the sequence of one member.
Then the category becomes convergence space over the set of arrows.
Such way ^{=unifies the nomenclature} of different mathematical regions - algebra and
topology.

A functor between two categories $f: X\doublerightarrow Y$ is defined as
a transport of
underlying graphs maintaining the composition of arrows
$$f(u\circ v)= f(u)\circ f(v)$$
and the appointment  of unit arrows
$$f(1_a)= 1_{f(a)}\tsk$$
Arbitrary  points in a category $X$ can be identified with
appointed unit arrow.
So the category entirely is defined by its arrows, and functors between
them coincide with continuous mappings for defined convergence of arrow's
sequences.

We can define a category of graphs $\GRPH$ compounded of all ^{graphs
=transports}. The points will be arbitrary graph and arrows will be
transports between such graphs.
Such transport  $f: X\doublerightarrow Y$ are defined as
an appointment  of vertexes $f_0: X_0\rightarrow Y_0$ and appointments
 of edges sets
 $$f_{x;y}: X(x;y)\rightarrow Y(f(x);f(y))\tsk$$
It can be concerned that the edges defines two different convergences for
sequences of one member, and mapping of vertexes are  continuous mappings
for both convergences.

 The composition of graph transports are defined in usual way
$$f\circ g (x)= g(f(x))\kbl f_{x,y}\circ g_{f(x),f(y)}=
(f\circ g)_{x,y}(g(f(x));g(f(y)))\tsk$$
The identity transport
$\Identity_X: X\doublerightarrow X$
is defined by identity  appointments
$$\Identity_X(x)= x\kbl (\Identity_X)_{x,y} = \Identity_{X(x;y)}\tsk$$
It will be units for  chosen composition of transports.

A Carte tensor product of two graphs $X\times Y$
in the category of graphs $\GRPH$
is defined by Carte tensor product for the sets of vertexes $X_0\times Y_0$
and the sets of edges $X\times Y$.
The source and target projections are also provided
by Carte tensor products
$$p_1\times p_1: X\times Y\rightarrow X_0\times Y_0 \kbl
p_2\times p_2: X\times Y \rightarrow X_0\times Y_0\tsk$$

So for the Carte tensor product of graphs $X\times Y$
we have edges  sets
$$X\times Y(\lan x,y\ran; \lan x',y'\ran )= X(x;x')\times Y(y;y')\tsk $$

It provides a bifunctor over the category of graphs $\GRPH$, but we shall
use only the functor $F: \GRPH\superrightarrow \GRPH$
which for the graph $X$ appoints tensor product $X\times T$ with
chosen ^{=assistant graph} $T$.

For a graphs transport $f: X\doublerightarrow Y$
we appoint another graphs transport
$$f\times \Identity_T : X\times T \doublerightarrow  Y\times T$$
taking the appointment for edges
$f\times \Identity_Y: X\times T\rightarrow Y\times Y$ and the appointment
 for  vertexes
$f_0\times \Identity_{X_0}: X_0\times T_0 \rightarrow Y_0\times T_0$.
We have checked in  the category $\SET$ that such appointments
maintains the arrows composition and unit arrows appointment.

We wish to define a joint pair of functors
$$\lan F,G\ran: \GRPH\rightleftarrows \GRPH \tsk$$
We need to construct an coadjoint exponential functor $G$.
For the graph $Y$ we provide the set $Y^T$
of all graphs transports $ \phi: T\doublerightarrow Y$. It will be
a set of vertexes  for a new graph. The edges will be defined by
transforms $\alpha: \phi\rightarrow   \psi$
between graphs transports $\phi,\psi: T\doublerightarrow Y$.
It is understood as a collection of edges in target graph $Y$
$$\alpha_t \in Y(\phi_0(t);\psi_0(t))\uparrow  t\in T_0\tsk$$
We shall work only with full collections of edges, but we also could work
with partial collection and get a more large exponential graph $X^T$.

The ^{unit =transform} $i: \Identity_{\GRPH}\rightarrow FG$  will be
 defined  only for graphs $X$ with chosen unit arrows $1_a\in X(a;a)$.
Also for assistant graph $T$ we demand to have chosen unit arrows
$1_s\in T(s;s)$.

We choose arbitrary edge  $1_a\in X(a;a)$ which will be called a unit arrow.
Such choosing  provides a  section
$\lambda_X(x): T\doublerightarrow X\times T$
with unanimously defined  edges appointment
$$\lambda_X(x)_u = \lan 1_x,u\ran \in X\times T \uparrow u\in T(s;t)\tsk$$
Choosing  an edge $1_t\in T(t;t)$ provides a
 graphs transport
$$\lambda_X: X\doublerightarrow (X\times T)^T $$
with unanimously defined edges appointment.
It for an  edge $\alpha\in X(a;b)$ will appoint the transform between
two sections
$$\Prod_{s\in T} \lan \alpha, 1_s\ran : \lambda_X(a)
\rightarrow \lambda_X(t)\tsk$$

A ^{unit =transform} will be defined  with  collection of
graphs transports
$$\lambda_X:  X\doublerightarrow (X\times T)^T\tsk$$
It for a  vertex $a\in X_0$
 appoints the section $\lambda_X(a):T \doublerightarrow X\times T$
with mapping  of vertexes $\lambda_X(a): T_0\rightarrow X_0\times T_0 $
$$\lambda_X(a)_t= \lan a,t\ran\in X_0\times T_0$$
and mapping of edges which for an edge $u\in T(s;t)$ appoints
the edge in the product of graphs
$$\lambda_X(a)_u= \lan 1_a,u \ran\in X\times T\tsk$$

For an edge $\alpha\in X(a,b) $ sections transport  appoints
the transform between sections
$$\Prod_{s\in T} \lan \alpha, 1_s\ran: \lambda_X(a)\rightarrow \lambda_X(b)$$
defined by collection of edges
$$\lan \alpha, 1_s \ran\in X\times T(
 \lan a,s\ran;\lan b,s\ran)= X(a;b)\times T(s;s)\tsk$$


A ^{counit =transform}  for taken joint pair
will be defined only for a graph $Y$ with chosen   mappings of
^{=diagonal arrows }
$$ Y(c;d)\times Y(d;e) \rightarrow Y(c;d)\circ Y(d;e)\subset
Y(c;e)\tsk$$
This transform will be  defined by collection of evaluation transports
$$\ev_Y:Y^T\times T\doublerightarrow Y \tsk$$
For the graphs transport $\phi: T\doublerightarrow Y$ and vertex $s\in T_0$
it appoints the vertex $\phi(s)\in Y_0$.
For the transform $\beta: \phi\rightarrow \psi$ and an edge $u\in T(s;t)$
it appoints the ^{=prediagonal arrow}

$$\alpha_s \circ \psi(u) \in Y(\phi_0(s);\psi_0(t))\tsk$$
$$\matrix { \phi_0(s) & &  \cr
      \mapdownk \alpha_s &\searrow    &  \cr
       \psi_0(s) & \maprightap \psi(u) &\psi_0(t) \cr}$$
\vskip \tarpas
So we have  got a joint pair
having  both unit transform and counit transform.
Nevertheless these transforms are only partial transforms, without
maintaining of arrows associative composition the evaluation
graphs transports
defined counit transform can't be  natural.
So we can't get natural bijection
between sets of graphs transports
$$\GRPH (X\times T; Y)=\rightarrow \GRPH (X; Y^T)\tsk$$

We shall prove the bijection only between the sets of special graphs
transports.


\Proposition
The choosing of unit arrows in the source  graph
$1_a\in X(a;a)$
and in an assistant graph $1_t\in T(t;t)$
allows us to define a name mapping
between the sets of graphs transports
$$\GRPH( X\times T;Y) \rightarrow  \GRPH(X;Y^T)\tsk$$

The choosing of diagonal arrows in the target graph $Y$ with composition
$$\circ : Y(c;d)\times Y(d;e)\rightarrow Y(c;e)$$
allows us to define a realization mapping
$$\GRPH (X;Y^T)\rightarrow \GRPH (X\times T;Y)\tsk$$

The name mapping is injective  over
graphs transports $\Phi:X\times T\doublerightarrow Y$
which are decomposable with  appointment of diagonal arrows  in the
target graph
$Y$
$$\Phi(\alpha,u)= \Phi(\alpha, 1_s)\circ \Phi(1_b, u)\uparrow
\alpha\in X(a;b), u\in T(s;t))\tsk$$
The realization mapping is injective over graphs transports
$\Psi: X\doublerightarrow Y^T$ which are neutral for choosing of
unit arrows in the source graph $X$ and assistant graph $T$
$$\Psi(1_a)_s\circ \Psi_0(a)_u= \Psi_0(a)_u \kbl$$
$$\Psi (\alpha)_s\circ
\Psi_0(b)_{1_s}= \Psi(\alpha)_s\tsk$$
\Proof:
For a graphs  transport
$\Phi: X\times T\doublerightarrow Y$
we shall construct its name $\Psi: X\doublerightarrow Y^T$.
For a vertex $a\in X_0$ it appoints graphs transport
$$\Psi(a): T\doublerightarrow Y$$
which for a vertex $t\in T_0$ appoints the vertex in the target graph
$$\Psi_0(a)_t= \Phi_0(a,t) \in Y_0$$
and for an edge $u\in T(s;t)$ it appoints the edge in the target graph
$$\Psi_0 (a)_u= \Phi (1_a, u)\in Y(\Phi_0(a,s);
\Phi_0(a,t))\tsk$$

For an edge $\alpha\in X(a;b)$ the new graphs transport
$ \Psi: X\doublerightarrow Y^T$ appoints the transform of graphs transports
$\Psi(\alpha):\Psi_0(a)\rightarrow \Psi_0(b)$ defined with collection
of edges
$$\Psi(\alpha)_t=\Phi(\alpha,1_t)\in Y( \Phi_0(a,t);\Phi_0(b,t))\tsk$$

Now for a graph transport $\Psi: X\doublerightarrow Y^T$ we shall
construct its realization
$\Phi:X\times T\doublerightarrow Y$.
For a vertexes $a\in X_0$ and $s\in T_0$ we appoint the
vertex in the target graph $Y$ which is got
as value  $\Psi_0(a)_s \in Y_0$
for  the graphs transport
$\Psi_0(a): T\doublerightarrow Y$.

For an edge in the Carte tensor product $\lan \alpha,u\ran \in
X(a;b)\times T(s;t) $ we appoint the diagonal edge
for graphs transform $\Psi(\alpha)_s\in
Y(\Psi_0(b)_s;\Psi_0(t)_s )$
and the edge appointed by graphs transport
$\Psi_0(b)_u
 \in Y(\Psi_0(b)_s;\Psi_0(b)_t)$
$$\Phi(\alpha,u)= \Psi(\alpha)_s\circ  \Psi_0(b)_u \in
Y(\Psi_0(a)_s;\Psi_0(b)_t)\tsk$$
%
In the Carte tensor product we have a natural appointment of
diagonal arrow
$$\lan \alpha,u\ran) = \lan \alpha,1_s\ran \circ \lan 1_b,u\ran
 \uparrow \alpha\in X(a;b), u\in T(s;t)\tsk$$
Let we have decomposable graphs
transform $\Phi:X\times T\doublerightarrow Y$
maintaining  such diagonal arrow
$$\Phi(\lan \alpha,u\ran)=\Phi(\lan \alpha,1_t\ran)\circ
\Phi(1_b,u\ran)\uparrow
\alpha\in X(a;b), u\in T(s;t)\tsk$$
Then for a name $\Psi:X\doublerightarrow Y^T$ we get the realization
$\Phi': X\times T\doublerightarrow Y$
equal to the same
graphs transform.
It for the arrows $\alpha\in X(a;b)$ and $u\in T(s;t)$ appoints
$$\Psi(\alpha)_s\circ \Psi_0(b)_u=\Phi(\lan \alpha,1_s\ran)
\circ \Phi (\lan 1_b, u\ran)=
\Phi(\lan \alpha,u\ran)\tsk$$

If we have equalities for the diagonal edges appointment
$$\Psi(\alpha)_s\circ\Psi_0(b)_{1_s}=
\Psi(\alpha)_s\kbl$$
$$\Psi(1_a)_s\circ \Psi_0(a)_u = \Psi_0(a)_u \kbl$$
then for its realization
$$\Phi(\lan\alpha,u\ran) = \Psi(\alpha)_s \circ \Psi_0(b)_u $$
we  get the  same name
$\Psi':X\doublerightarrow Y^T$
$$\Psi'_0(a)_u= \Phi(\lan 1_a, u\ran)=\Psi(1_a)_s\circ \Psi_0(a)_u =
\Psi_0(a)_u$$
and
$$\Psi'(\alpha)_s=\Phi (\lan \alpha, 1_s\ran = \Psi(\alpha)_s
\circ \Psi_0(b)_{1_s}=
\Psi(\alpha)_s \tsk$$

\irodymopabaiga

We shall provide another proving of this proposition with standard tools
in general categories. First we shall check that realization will reverse the
name mapping. For this we shall construct commuting diagram
$$\matrix{
X\times T & \mapright\lambda_X\times 1_T &(X\times T)^T\times T &
\mapright  f^T\times 1_T & Y^T\times T \cr
& \searrow &\mapdownd \ev_{X\times T} & &\mapdownd\ev_Y \cr
&&X\times T&\maprightap f & Y \cr}$$
\vskip\tarpas
We get the evaluation in the space $X\times T$  by choosing composition
$$\lan\alpha, 1_s\ran \circ \lan 1_b,u\ran =
\lan\alpha,u\ran \in X(a;b)\times T(s;t)$$
 for arbitrary $\alpha\in X(a;b)$ and $u\in T(s;t)$.

This is natural choice, but we need to check that with such choice we have 
got a  commuting diagram.


At first we shall check the first triangular equality for arbitrary graphs
$X$ and $T$ with chosen unit arrows $1_a\in X(a;a)$ and $1_t\in T(t;t)$.
We must prove the identic transport for composition of graphs transports
\vskip\tarpas
$$X\times T\mapright \lambda_X\times 1_T (X\times T )^T\times T
\mapright \ev_{(X\times T)}  X\times T \tsk$$

We have projection of categories $\GRPH\superrightarrow \SET $
which for a graph $X$ appoints its vertexes set $X_0$, and for a graphs
transport $f: X\doublerightarrow Y$ appoints the vertexes  appointment
$f_0:X_0\rightarrow Y_0$.

 The  constructed Carte tensor product of graphs   $X\times Y$
is projected to the
Carte tensor product of sets $X_0\times Y_0$, i. e. we have commuting
diagram of functors

$$\matrix { \GRPH \times \GRPH & \mapright X\times Y & \GRPH \cr
     \downarrow  & &\downarrow \cr
         \SET\times \SET & \maprightap X_0\times Y_0 & \SET \cr} $$
 \vskip \tarpas
For an exponential graph $Y^T$ such projections appoints the set of all
graphs transports $\phi: T\doublerightarrow Y$.
It will be a primary projection.
            So we get the composition of vertexes appointments
$$X_0\times T_0\mapright (\lambda_X)_0\times 1_{T_0}
((X\times T)^T)_0\times T_0
\mapright (\ev_{(X\times T)})_0 X_0\times T_0 \tsk$$

The secondary projection is defined with
deformation  of each graphs transport $\phi: T\doublerightarrow Y$ to its
vertexes appointment $\phi_0: T_0\rightarrow Y_0$. We shall need
to calculate these projections only for some concrete graphs transports.
For the secondary projection we get composition  of appointments
$$X_0\times T_0\mapright \lambda_{X_0}\times 1_{T_0}
(X_0\times T_0)^{T_0} \times T_0 \mapright \ev_{(X_0\times T_0)}
X_0\times T_0 \kbl$$
which is equal to identity appointment by
 the first triangular equality
in the category of sets $\SET$.

The evaluation appointment for a couple $ \lan\phi,s\ran\in Y^T_0\times T_0$
appoints the
value $\phi_0(s)\in Y_0$, therefore  for arbitrary
transport $\phi: T\doublerightarrow X\times T$  it depends only from
its projection $\phi_0: T_0\rightarrow X_0\times T_0$.
So we have get the first triangular
equality also for the primary projection.

It rests to check the first triangular equality only for edges appointments.
For a couple of  edges $\alpha\in X(a;b)$ and $u\in T(s;t)$
the first transport
$$\lambda_X\times \Identity_T: X\times T\doublerightarrow (X\times T)^T\times T $$
will appoint the couple of transform between two sections
$$\Prod_{s'\in T} \lan \alpha, 1_{s'} \ran :
\lambda_X(a)\rightarrow \lambda_X(b)$$
 and the same edge $u\in T(s;t)$,
Further the  evaluation transport in the space $X\times T$
$$\ev_{X\times T}: (X\times T)^T\times T\doublerightarrow X\times T $$
will appoint the  diagonal arrow
$$\lan \alpha,1_s\ran \circ \lan 1_b, u\ran =
 \lan \alpha, u\ran \in X(a;b)\times T(s;t)\tsk$$
So we get the same couple of edges $\alpha\in X(a;b)$ and $u\in T(s;u)$,
and we end the checking of the first triangular equality for graphs.

Now we shall check for what graphs transport $f: X\times T\doublerightarrow Y$
we have commuting quadrat with a transform
$$\Prod_{s'\in T}  \lan \alpha, 1_{s'}\ran : \lambda_X(a)\rightarrow
\lambda_X( b) $$   between two sections
$\lambda_X(a), \lambda_X(b)\in (X\times T)^T$
$$ \matrix{ (X\times T)^T\times T  & \mapright f^T\times 1_T & Y^T\times T \cr
     \mapdownk \ev_{(X\times T)} & & \mapdownd \ev_Y \cr
     X\times T & \maprightap f & Y \cr }$$
\vskip\tarpas
Let we have decomposable transport $f: X\times T\doublerightarrow Y$
$$f(\alpha, u )= f(\alpha, 1_s)\circ f(1_b, u) \in
Y(f_0(a,s);f_0(1_b,u))\tsk$$

Then the first evaluation $\ev_{(X\times T)}$  for the couple of
transform between sections $\Prod_{s'\in T} \lan \alpha, 1_{s'}\ran:
\lambda_X(a)\rightarrow \lambda_X(b)$ and the edge $u\in T(s;t)$
will appoint  the diagonal arrow
$$\lan \alpha,1_s\ran\circ \lambda_X(b)_u=
\lan \alpha, 1_s\ran \circ \lan 1_b, u\ran =\lan \alpha,u\ran $$
and  the  transport $f: X\times T\doublerightarrow Y$ will appoint
the value
$$ f(\alpha,u)\in Y(f_0(a,s);f_0(b,t))\tsk$$

Changing of target space with decomposable transport
$f:X\times T\rightarrow Y$ for the transform between sections
$\Prod_{s'\in T} \lan \alpha, 1_{s'}\ran: \lambda_X(a)\rightarrow \lambda_X(b)$
will appoint the transform between changed sections
$$\Prod_{s'\in T} f(\alpha, 1_{s'}): \lambda_X(a)\circ f\rightarrow \lambda_X(b)
\circ f \kbl$$
so the evaluation transport for the couple of such transform and the same edge
$u\in T(s;t)$ will appoint the same diagonal arrow
$$f(\alpha, 1_s)\circ f(\lambda_Y(b)_u)=
f(\alpha, 1_s)\circ f(1_b, u)= f(\alpha,u)\tsk$$

Now we shall check that the name mapping reverses the realization.
For this we shall construct another commuting diagram
$$\matrix{Y^T & \mapleft (\ev_Y)^T & (Y^T\times T)^T &\mapleft (g\times 1_T)^T & (X\times T)^T \cr
&\nwarrow & \mapupd\lambda_{Y^T} & & \mapupd\lambda_X \cr
& & Y^T& \mapleft g & X \cr }$$
\vskip\tarpas
In the graph $Y$ we have diagonal arrows mapping 
$$\circ: Y(c;d)\times Yd;e)\rightarrow Y(c;e)\kbl $$
but for a sections transport $\lambda_{Y^T}$ we need to choose the unit arrows
in exponential graph $Y^T$. It will be defined with collection of unit arrows
images only
for image vertexes
$$ g_{a,a}(1_a)\in Y^T(g_0(a);g_0(a))\tsk$$

We shall check the second triangular  equality as an
identity transform by composition
$$Y^T \mapright \lambda_{Y^T} (Y^T\times T)^T \mapright (\ev_Y)^T  Y^T \tsk$$
begun  with taken  transport $g: X\doublerightarrow Y^T$
                                                      having the neutral properties
for images of unit arrows from the source graph
$1_a\in X(a;a)$ and assistant graph $1_s\in T(s;s) $
$$g(1_a)_s \circ g_0(a)_u =g_0(a)_u \in Y(g_0(a)_s;g_0(a)_t)
\uparrow u\in T(s;t)\kbl$$
$$g(\alpha) _s\circ g_0(b)_{1_s} = g(\alpha)_s \in Y(g_0(a);g_0(b)_s)
\uparrow \alpha\in X(a;b)\tsk$$

The sections transport
$\lambda_{Y^T}: Y^T\doublerightarrow (Y^T\times T)^T $
will be defined using the images of chosen unit  arrows
$g_0(1_a): g_0(a)\rightarrow g_0(a)$. We use a  notation for edges in
assistant graph  $u\in T(s;t)$. But for the same  repeated
graph $T$ we apply a new notation  $u'\in T(s';t')$.

First we shall check the second triangular equality
with the primary  projection for the set of all graph transports
$(Y^T)_0= \lbrace \phi: T\doublerightarrow  Y\rbrace $
in the category of sets $\SET$
$$(Y^T)_0\mapright (\lambda_{(Y^T)})_0 ((Y^T \times T)^T)_0 \mapright
(\ev_{Y^T}^T)_0  (Y^T)_0 $$
begun with the appointment of taken graphs transport
$$g_0: X_0 \rightarrow (Y^T)_0 \tsk$$
For sections transport $\lambda_{Y^T}: Y^T\doublerightarrow (Y^T\times T)^T$
we take vertexes appointment
$\lambda_{Y^T}: (Y^T)_0\rightarrow ((Y^T \times T)^T)_0$
which for a graphs transport
$\phi:T\doublerightarrow Y$ appoints another graphs transport
$$\lambda_{(Y^T)}(\phi): T\doublerightarrow Y^T\times T \tsk$$
We can apply the secondary projection  to get a new triangular equality
for the same graphs transform $\phi: T\doublerightarrow Y$, but
with  a new sections appointment in the category of sets $\SET$
$$(Y^T)_0\mapright \lambda_{(Y^T)_0} ((Y^T)_0 \times T_0)^{T_0} \mapright
(\ev_{(Y^T)_0})^{T_0}  (Y^T)_0 \tsk$$
It for a graphs transport $\phi: T\doublerightarrow Y$ will appoint
the section in the category of sets
$$\lambda_{(Y^T)_0}(\phi): T_0\rightarrow (Y^T)_0\times T_0 $$
which for a vertex $t\in T_0$ appoints the couple $\lan \phi, t\ran \in
(Y^T)_0\times T_0$.

For the set of all appointments $\phi: T_0\rightarrow Y_0$ we have  already the
second triangular equality
$$(Y_0)^{T_0}\mapright  \lambda_{(Y_0)^{T_0}} ((Y_0)^{T_0}\times T_0)^{T_0}
\mapright (\ev_{(Y_0)})^{T_0}  (Y_0)^{T_0}\tsk$$
The first arrow is a sections
appointment defined  for arbitrary appointment $\phi: T_0\rightarrow Y_0$
$$\lambda_{(Y_0)^{T_0}}:T_0\rightarrow (Y_0)^{T_0} \times T_0 $$
So the triangular equality  remains valid also for an imbedded smaller set
$(Y^T)_0\subset (Y_0)^{T_0}$ of all appointments get from
graphs transports $\phi: T\doublerightarrow Y$.

This new triangular equality  will provides also the triangular
equality for the primary projection.
It rests to check 
the changing of target space  with evaluation transport
$$(\ev_Y)^T: (Y^T\times T)^T \doublerightarrow Y^T$$
only for edges $u'\in T(s';t')$.
 The section $\lambda_{Y^T}(g_0(a)): T\doublerightarrow Y^T\times T$
for arbitrary   edge $u'\in T(s';t')$ will appoint the
edge between couples
$$ \lan g_{a,a}(1_a), u' \ran : \lan g(a),s'\ran \rightarrow  \lan g(a),t'\ran $$
defined with the image of unit arrows  in source graph $1_a\in X(a;a)$.
Further evaluation transport
$\ev_Y: Y^T\times T\doublerightarrow Y$ will provide
the diagonal arrow
$$g_a,a(1_a)_{s'}\circ g_0(a)_{u'} \in Y(g_0(a)_{s'};g_0(a)_{t'})$$
equal by the  neutral property to the same edge appointed by taken transport
$g(a)\in Y^T$
$$g_{a,a}(1_a)_{s'}\circ g_0(a)_{u'} = g_0(a)_{u'}\in
Y(g_0(a)_{s'};g_0(a)_{t'})\tsk$$
So we have got the same graphs transport $g(a)$.

Finally we need to check the second triangular equality for the edges
appointments. By the graphs transport     $g: X\doublerightarrow Y^T$
the edge $\alpha\in X(a;b)$ will be appointed to the transform
$$g(\alpha): g_0(a )\rightarrow g_0(b)$$
defined with collection of edges $g(\alpha)_s\in Y(g_0(a)_s;g_0(b)_s)$.
The  sections transport
$\lambda_{Y^T} : Y^T\doublerightarrow (Y^T\times T)^T$
for such transform will be fully defined with chosen unit arrows
in assistant graph $1_{s'}\in T(s';s')$.
The transform  between sections
$$\lambda_{Y^T}(g(\alpha)): \lambda_{Y^T} (g_0(a))\rightarrow
\lambda_{Y^T} (g_0(b)) $$
will be defined with collection of edges in  the product of graphs
$$\lambda_{Y^T} (g(\alpha))_{s'}= \lan g(\alpha),1_{s'}\ran:
\lan g_0(a),s'\ran \rightarrow
 \lan g_0(b),s'\ran \tsk$$

Further we shall check the changing of target space with evaluation transport
$$(\ev_Y)^T: (Y^T\times T)^T\doublerightarrow Y^T \tsk$$
The evaluation transport $\ev_Y: Y^T\doublerightarrow Y$
for the couple $\lan g(\alpha),1_{s'} $ 
will appoint the
diagonal arrow
$$g(\alpha)_{s'}\circ g_0(b)_{1_{s'}} \in Y(g_0(a)_s;g_0(b)_s)$$
By the neutral property of chosen unit arrows in assistant graph
$1_{s'}\in T(s';s') $ we have equality
$$g(\alpha)_{s'}\circ g_0(b)_{1_{s'}}
= g(\alpha)_{s'} \tsk$$
So we have got the same transform between taken graphs transports
$$g(\alpha)= \Prod_{s'\in T_0} g(\alpha)_{s'} \in Y^T(g_0(a);g_0(b))\tsk$$
We have finally shown the second triangular equality begun with taken
graphs transport
$g: X\doublerightarrow Y^T$.

Now we shall check the commuting quadrat
between defined sections mappings
$$ \matrix { (Y^T\times T)^T  &
\mapleft (g\times 1_T)^T & (X\times T)^T \cr
 \mapupd \lambda_{Y^T} &   & \mapupd \lambda_X \cr
 Y^T & \mapleftap g & X\cr } $$
\vskip\tarpas
For a vertex $a\in X_0$ we appoint the graphs transport $g_0(a)\in Y^T$
which provides the section $\lambda_{Y^T}(g_0(a)): T\doublerightarrow Y^T\times T$
 which for a vertex  $s'\in T_0$ appoints the couple $\lan g_0(a), s'\ran$
and for an edge $u'\in T(s';t')$ appoints the transform between sections
$$\lan g(1_a), u'\ran : \lan g_0(a),s'\ran \rightarrow
\lan g_0(a),t'\ran \tsk$$
We get the same sections and their transforms
also by graphs transport
$$(g\times \Identity_T)^T: (X\times T)^T
 \doublerightarrow ( Y^T\times T)^T \tsk$$
For an edge $\alpha\in X(a;b)$ taken graphs transport will appoint the
transform between two graphs transports
$g(\alpha): g_0(a)\rightarrow g_0(b)$, and sections transport provides
the transform between two sections defined with edges in the product
of graphs $Y^T \times T$
$$\lan g(\alpha), 1_{s'} \ran: \lan g_0(a), s'\ran \rightarrow
\lan g_0(b), s'\ran \tsk$$
This ends another more categorical proving of former proposition.
\vskip\tarpas

Choosing of diagonal arrows mappings in the target graph $Y$ provides
a possibility
to have another exponential superfunctor. For two graphs transports
$\phi,\psi: T\doublerightarrow Y$ we appoint the set
of natural transforms $\alpha: \phi\rightarrow \psi$.
We will adapt a new
notation for such graph $Y^{(T)}$.

Evaluation transport can be defined in
two different ways. For the couple of a transform
$\alpha: \phi\rightarrow \psi$ between to graphs transports
$\phi, \psi: T\doublerightarrow  Y$ and an edge between two vertexes in
source graph $u\in T(s;t)$  we have defined ^{prediagonal =arrow }
$$\ev_{Y}^+(\lan \alpha,u\ran )= \alpha_s\circ \psi_{s,t}(u)\kbl$$
and now we can define another ^{postdiagonal =arrow}
$$\ev_Y^- (\lan \alpha, u\ran) = \phi_{s,t}(u)\circ \alpha_t \tsk$$
I haven't find another names in English. It may be similar
to using of names ^{=prefix} and ^{=suffix}. A transform
$\alpha: \phi\rightarrow \psi$  is called ^{=natural} if we get
commuting  quadrats from equality of prediagonal and postdiagonal
arrows
$$\alpha_s \circ \psi_0(u)= \phi_0(u)\circ \alpha_t\tsk$$
\vskip\tarpas
$$\matrix { \phi_0(s) &\mapright \phi_{s,t}(u) & \psi_0(t) \cr
           \mapdownk \alpha_s & \searrow  & \mapdownd \alpha_t \cr
           \psi_0(s) & \maprightap \psi_{s,t}(u) & \psi_0(t) \cr } $$
\vskip\tarpas
We wish to define the new exponential space $Y^{(T)}$ in more categorical
way. We have two evaluation arrows. One is for ^{=preevalution}
$$\ev_Y^+: \prod_{s\in T_0} Y(\phi_0(s); \psi_0(s))
\times T(s;t)\rightarrow
$$$$Y(\phi_0(s);\psi_0(s))\times T(s;t) \rightarrow Y(\phi_0(s);\psi_0(t)) \kbl$$
and another is for ^{=postevaluation }
$$\ev_Y^-: \prod_{s\in T_0} Y(\phi_0(s); \psi_0(s))
\times T(s;t)\rightarrow
$$$$Y(\phi_0(t);\psi_0(t))\times T(s;t) \rightarrow Y(\phi_0(s);\psi_0(t)) \kbl$$
Using the names of such mappings we get new mappings
to the functional space defined in closed category $\SET$
$$\Prod_{s\in T_0} Y(\phi_0(s);\psi_0(s))\tworightarrows
Y(\phi_0(s);\psi_0(t))^{T(s;t)} \tsk$$
Their product for all couples $s,t\in T_0$ provides equalizer coinciding
with new space of natural transforms
$$\rightarrow Y^{(T)} \rightarrow \Prod_{s\in T_0} Y(\phi_0(s);\psi_0(t))
\tworightarrows \Prod_{s,t\in T_0} Y(\phi_0(s);\psi(t))^{T(s;t)} \tsk$$
For graphs transports $g:X\doublerightarrow Y^T$ we get different realization
$$f= (g\times \Identity_T)\circ \ev_Y^\pm : X\times T\doublerightarrow Y\tsk$$
Preevaluation arrows define ^{=prerealization}, and postevaluation arrows
provide ^{=postrealization}. The name mapping
$$g= \lambda_X\circ f^T: X\doublerightarrow Y^T$$
remains the same for both evaluation arrows.

We repeat former proposition for the exponential set of natural transforms.
             We shall say that graphs transport $\Phi: X\times T\doublerightarrow Y$
to the target space $Y$ with diagonal arrows mappings
$$\circ : Y(a;b)\times Y(b;c)\rightarrow Y(a;c)$$
is
^{=predecomposable} if we have an equality
$$\Phi(\alpha, 1_s)\circ \Phi(1_b, u)=
\Phi(\alpha,u)\uparrow
\alpha\in X(a;b), u\in T(s;t)$$
and ^{=postdecomposable}  if we have another equality
$$\Phi(\alpha,u)= \Phi(1_a,u)\circ \Phi(\alpha, 1_t )
\uparrow
\alpha\in X(a;b), u\in T(s;t)$$
The graphs transport will be called ^{=decomposable} if it
is predecomposable and postdecomposable.

We shall say that graphs transport $\Psi X\doublerightarrow Y^T$ is
^{=preneutral} for chosen unit arrows in source graph $1_a\in X(a;a)$
and assistant graph $1_s\in T(s;s)$
if we have equalities
$$\Psi (\alpha)_s\circ \Psi_0(b)_{1_s}= \Psi(\alpha)_s
 \kbl$$
$$\Psi(1_a)_s\circ \Psi_0(a)_u= \Psi_0(a)_u \tsk$$
And we shall say that such graphs transport is ^{=postneutral}
if we have another equalities
$$ \Psi(\alpha)_s= \Psi_0(a_{1_s}\circ \psi(\alpha_s\kbl $$
     $$ \Psi_0(a)_u = \Psi_0(a)_u\circ \Psi(1_a)_t \tsk$$
The graphs transport will be called ^{=neutral} for chosen unit arrows in
source graph and assistant graph if it is preneutral and postneutral.

\Proposition
The choosing  of unit arrows in a source graph $1_a\in X(a;a)$
and  in an assistant graph $1_s\in T(s;s)$  allows us to
define the name mapping between the sets of graphs transports
$$\GRPH( X\times T;Y) \rightarrow  \GRPH(X;Y^T)\tsk$$

For a  diagonal edges mapping in a target graph $Y$
$$\circ : Y(c;d)\times Y(d;e)\rightarrow Y(c;e)$$
the  choosing of evaluation transport defined with prediagonal or postdiagonal
arrow allows us to define the realization mapping
$$\GRPH (X;Y^T)\rightarrow \GRPH (X\times T;Y)\tsk$$

The name of  graphs transport
$\Phi:X\times T\doublerightarrow Y$
which is  predecomposable and postdecomposable for diagonal arrows  mappings
in the target graph  $Y$
$$\Phi(\alpha, 1_s)\circ \Phi(1_b, u)=
\Phi(\alpha,u)= \Phi(1_a,u)\circ \Phi(\alpha, 1_t )
\uparrow
\alpha\in X(a;b), u\in T(s;t)$$
is corestrained in exponential graph of natural transforms  $Y^{(T)}$.

The name mapping  is injective over such graphs transports
$$\GRPH(X\times T; Y) \rightarrow \GRPH (X; Y^{(T)}) \tsk$$

The realization mapping  coincides over graphs transports corestrained
in the exponential graph of natural transforms
 $\Psi: X\doublerightarrow Y^{(T)}$
for both prediagonal or postdiagonal arrows
and it is injective if taken graphs transport
$\Psi: X\doublerightarrow Y^{(T)}$ is  preneutral and postneutral
for choosing of
unit arrows in the source graph $X$  and  the assistant graph $T$
$$\Psi (\alpha)_s\circ \Psi_0(b)_{1_s}= \Psi(\alpha)_s=
\Psi_0(a)_{1_s}\circ \Psi(\alpha)_s \kbl$$
$$\Psi(1_a)_s\circ \Psi_0(a)_u= \Psi_0(a)_u = \Psi_0(a)_u\circ \Psi(1_a)_t
\tsk$$
\Proof:
We present the more detailed categorical proving of such proposition.

First we notice that the name of graphs transport
$f: X\times T\doublerightarrow  Y$
 is defined using sections transport
$\lambda_X: X\doublerightarrow (X\times T)^T $
$$g= \lambda_X\circ f^T :  X\doublerightarrow  Y^T \tsk$$
For predecomposable graphs transport $f: X\times T\doublerightarrow Y$
the prerealization reverses its name. So the name mapping will be injective
over the set of predecomposable graphs transports and prerealization
mapping covers this set.

The same is true for the set of postdecomposable graphs transports. The
name mapping is injective and postrealization mapping covers this set.

The name of decomposable graphs transport
$f: X\times T \doublerightarrow Y$ is included in the exponential
space of natural transforms $Y^{(T)}$.

Having commuting  diagrams  with  preevaluation or
postevaluation transports
$$\matrix { X\times T & \mapright \lambda_X\times 1_T  &
 (X\times T)^T \times T  & \mapright f^T\times 1_T & Y^T \times T \cr
%
&\searrow &\mapdownd \ev^\pm_{(X\times T)}  & &\mapdownd \ev^\pm_Y  \cr
%
& &X\times T  & \maprightap f & Y\cr}$$
\vskip \tarpas
we shall check  the ^{=corestriction}  of name
$$g: X\mapright \lambda_X (X\times T)^T \mapright f^T  Y^T \tsk$$
in exponential space of natural transforms  $ Y^{(T)}$.

For a vertex $a\in X_0$ it appoints the section
$\lambda_X(a): T\doublerightarrow  X\times T$ which for an edge
$u\in T(s;t)$ appoints the couple of edges
$$\lan 1_a,u\ran : \lan a,s\ran \rightarrow \lan a,t\ran $$
between the couples of vertexes $\lan a,s\ran\in X_0\times T_0$ and
$\lan a,t\ran\in X_0\times T_0$.
Further the changing of target space by graphs
transport $f: X\times T\doublerightarrow Y$ will appoint a graphs
transport  $T\doublerightarrow Y$ which for the edge $u\in T(s;t)$
will appoint the edge  between vertexes in target space $Y$
$$f(1_a,u): f_0(a,s) \rightarrow f_0(a,t) \tsk$$

For an edge in source space $\alpha\in X(a;b)$ we get the transform between
sections
$\lambda_X(\alpha): \lambda_X(a)\rightarrow \lambda_X(b)$ defined with
collection  of couples of edges
$$\lan \alpha,1_s\ran : \lan a,s\ran \rightarrow \lan b,s\ran \uparrow
s\in T_0\tsk$$
Further by changing of target space with graphs transport
$f: X\times T\doublerightarrow Y$  we get transform  between earlier
graphs transports $T\doublerightarrow Y$ defined with collection of
edges
$$f(\alpha,1_s): f_0(a,s)\rightarrow f_0(b,t) \tsk$$
Such transform will be neutral if we should have commuting diagrams
$$\matrix {f_0( a,s) &  \mapright f(1_a,u) & f_0(a,t)\cr
          \mapdownk f(\alpha,1_s) & & \mapdownd f(\alpha, 1_t) \cr
          f_0(b, s) & \maprightap f(1_b,u)  & f_0(b, 1_t ) \cr }$$
\vskip\tarpas
This is proved by diagonal arrows mappings
$$\matrix {f_0( a,s) &  \mapright f(1_a,u) & f_0(a,t)\cr
          \mapdownk f(\alpha,1_s) &\searrow  & \mapdownd f(\alpha, 1_t) \cr
          f_0(b, s) & \maprightap f(1_b,u)  & f_0(b, 1_t ) \cr }$$
\vskip\tarpas
Such diagonal arrow is provided by
$f(\alpha,u): f_0(a,s)\rightarrow f_0(b,t)$
from commuting diagrams drown for both evaluation transports $\ev^\pm_Y$, i. e.
we have equalities  for prediagonal and postdiagonal arrows
$$ f(\alpha,1_s)\circ f(1_b, u)= f(\alpha,u)= f(1_a,u)\circ f(\alpha,1_t)
\tsk$$

Finally we need to check that for a graphs transport
$g: X\doublerightarrow Y^T$
with neutral properties we get injective  realization mapping
$$ \GRPH(X;Y^{(T)})\rightarrow \GRPH(X\times T;Y)\tsk$$

 First we can notice that both prerealization and postrealization
 coincides over graphs transports corestricted in exponential space
of natural transforms. Such realizations  are
defined by composition of graphs transports

$$ f: X\times T \mapright g Y^T\times T \mapright {\ev_Y^\pm}  Y\tsk$$
For the natural transform both evaluation transports appoints the same diagonal
arrow as
for the graphs transports corestricted in exponential space of natural
transforms $g: X\doublerightarrow Y^{(T)}$  both preneutral and
postneutral properties coincide.
$$ \matrix { g_0(a)_s & \mapright g_0(a)_{1_s} & g_0(a)_s \cr
\mapdownk g(\alpha)_s & \searrow & \mapdownd g(\alpha) _s \cr
g_0(b)_{1_s}  & \maprightap g_0(b)_{1_s} & g_0(b)_s \cr } \hskip 10 pt
\matrix { g_0(a) & \mapright g_0(a)_u & g_0(a)_t \cr
\mapdownk g(1_a)_s & \searrow  & \mapdownd g(1_a)_t \cr
g_0(a)_s  & \maprightap g_0(a)_u  & g_0(a)_t \cr } $$
\vskip \tarpas

Taking one of neutral properties, for example preneutral one,
we get  injective realization mapping over exponential space of
natural transforms.

\irodymopabaiga

Later we could  want to work  with categories
having weakly associative composition of arrows, i. e. with natural
isomorphisms
$$S_{\alpha,\beta,\gamma}:\alpha\circ(\beta\circ \gamma)\rightarrow
(\alpha\circ \beta) \circ \gamma \tsk$$

If we should work with graphs transforms $\Phi: X\times T\doublerightarrow Y$
which maintain both arrow composition
$$ \Phi(1_a,u)\circ \Phi(\alpha,1_t)=
\Phi(\alpha,u) = \Phi(\alpha, 1_s)\circ
\Phi(1_b,u)\kbl$$
then we could  work only with natural transforms
between graphs transforms $\phi,\psi: T\doublerightarrow Y$
to get a smaller exponential
graph $Y^{(T)}$.
The evaluation transport for such nonassociative arrows composition
doesn't maintain the arrows composition,
but it  is not difficult to calculate the isomorphism for
evaluation transport $Y^T\times T\doublerightarrow Y$
$$\ev_Y(\alpha\circ \beta, u\circ v) \rightarrow
 \ev_Y(\alpha,u) \circ \ev_Y(\beta,v)\tsk$$
So we can apply former proposition to get bijection between
arrows sets in such categories
$$\GRPH (X\times T;Y)=\rightarrow \GRPH(X; Y^{(T)})\tsk$$

\vskip\tarpas
Next we shall define an exponential superfunctor in the  category of
all categories $\CAT$.
The points in this category will be all possible categories.
We define a category  $X$ as the graph with the set  $X$ of edges
 coinciding with the set of category's arrows  and the set $X_0$
 of vertexes coinciding with the set of category's points.
We have arrows composition
$$\circ : X(a;b)\times X(b;c)\rightarrow X(a;c)$$
with associativity equality
$$f\circ (g\circ h)= (f\circ g) \circ h\uparrow f\in X(a;b), g\in X(b;c),
h\in X(c;d)\tsk$$
Also we have unit arrows $1_a\in X(a;a)$ which are ^{=preneutral} and
^{=postneutral} for arrows composition
$$1_a\circ f= f= f\circ 1_b \uparrow f\in X(a;b)\tsk$$

The arrows sets in the category of categories $\CAT(X;Y)$
will be compounded of all possible functors
$f: X\doublerightarrow Y$ between two categories $X$ and $Y$.
They will be defined by transport of graphs with two appointments. One for
the set of edges     $f: X\rightarrow Y$, and another for
the set of vertexes
$f_0: X_0\rightarrow Y_0$.
The arrows appointment is defined with collection of  mappings for
arrows sets between two points
$$f_{a,b}: X(a;b)\rightarrow  Y(f(a);f(B))\tsk$$

The functor must maintain the composition of arrows
$$f_{a,c} (\alpha\circ\beta)= f_{a,b} (\alpha)\circ f_{b,c} (\beta)
\uparrow \alpha\in X(a;b), \beta\in X(b;c) \tsk$$
Also it must maintain unit arrows
$$f_{a,a} (1_a)= 1_{f(a)} \tsk$$

Functors between  the categories can be understood as continuous transports
between graphs with convergence defined by composition of arrows and
appointment of unit arrows. It also can be considered as continuous mapping
between the sets of points with additional convergences defined by edges
between such points.
It will be helpful when we want to imagine
 more tremendous
construction such as superfunctors.

The  superfunctors  will be usual functors,  only  defined on
larger category.
It can be imagined as a functor over
the category of convergence spaces compounded with all continuous mappings.
A superfunctor $F$ for the category $X$ will appoint another
category $X^F$, and  it
defines mappings over the sets  of functors
$$F_{X,Y}:\CAT(X;Y)\rightarrow \CAT(X^F;Y^F)\tsk$$
It must maintain the composition of functors
$$(f\circ g)^F= f^F\circ g^F$$
and the appointment of identity functors $\Identity_X: X\doublerightarrow X$
$$(\Identity_X)^F= \Identity _{(X^F)}\tsk$$

We shall be interested in some concrete superfunctors
$$F: \CAT \superrightarrow \CAT \tsk$$

The first example of superfunctor is provided  with a ^{Carte tensor =product}
of two  categories.
A Carte tensor product of two categories $X\times Y$ is defined on the
Carte tensor product of graphs, i. e.  we  have  the Carte tensor product
for the sets of vertexes $X_0\times Y_0$  and the Carte tensor product
for the
sets of arrows $X\times Y$. Source and target projections are
defined with Carte product of correspondent projections
$$p_1\times p_1: X\times Y\rightarrow X_0\times Y_0\kbl
p_2\times p_2: X\times Y \rightarrow X_0\times Y_0 \tsk$$

The arrows composition and appointment of unit arrows  are also defined
as Carte products
$$(X\times Y(\lan x,y\ran; \lan x',y'\ran)) \times (X\times Y (\lan x',y'\ran;
\lan x'',y''\ran))\rightarrow X\times Y(\lan x,y\ran; \lan x'',y''
 \ran )\kbl$$
$$ 1_{\lan x,y\ran} = 1_x\times 1_y \tsk$$

This is an instance of general construction of Carte tensor product in
convergence spaces.

For chosen assistant category $T$ we get  a superfunctor
in the category $\CAT$ of categories.
For arbitrary category $X$ we appoint the Carte tensor product
$X\times A$ and for arbitrary functor $f: X\doublerightarrow X'$ we appoint
the Carte tensor product with identity functor of assistant category
$f\times \Identity_T: X\times A\doublerightarrow X'\times T$.

We shall try to define a coadjoint  ^{=exponential superfunctor}.
For a category $Y^T$ we take a set  of all possible functors
$\phi:T\doublerightarrow Y$ as a set of points, and a set
of all possible natural transformations
$\phi\rightarrow \psi$  as a set of arrows
between two functors
$\phi,\psi: T\doublerightarrow Y$.
The ^{natural =transform}  is  defined with collection of arrows
in the target category
$$\phi(s)\rightarrow \psi(s)\in Y$$
which meets the
coherence conditions of ^{commuting =diagrams} for arbitrary
arrow in source category $u\in T(s;t)$
$$\matrix{ \phi(s) & \mapright {\phi(u)} &\phi (t) \cr
           \downarrow  &   &\downarrow \cr
           \psi(s) & \maprightap {\psi(u)} &\psi(t)\cr}\tsk$$
\vskip \tarpas
The composition of  transforms $\phi\rightarrow \psi$ and
$\psi\rightarrow \xi$
is defined over each point $s\in T$
$$\phi(s)\rightarrow \psi(s)\rightarrow \xi(s) \tsk$$
Easy to see that such composition maintains the property of commuting
diagrams.  The most easy way it to do is a ^{=chasing correspondent diagrams}.
This can be also interpreted as a property of continuous transforms.

Having commuting quadrats  for arbitrary edge in assistant category
$u\in T(s;t)$
$$\phi(u)\circ \alpha_t= \alpha_s\circ \psi(u)\kbl$$$$
\psi(u)\circ \beta_t= \beta_s\circ \xi(u)\kbl$$
we get a new commuting quadrat
$$\phi(u)\circ (\alpha_t\circ \beta_t)= (*\alpha_s\circ \beta_s)\circ \xi(u)
\tsk$$
$$\matrix {
\phi_0(s)  & \mapright \alpha_s & \psi_0(s) & \mapright \beta_s  & \xi_0(s)\cr
\mapdownk \phi(u) &  & \mapdownk \psi(u) & & \mapdownd \xi(u)  \cr
\phi_0(t) & \maprightap \alpha_t & \psi_0(t) & \maprightap \beta_t
 & \xi_0(t)  \cr } $$
\vskip \tarpas
The  proving  uses three ways from a vertex $\phi_0(s)$ to the vertex
$\psi_0(t)$
$$(\alpha_s\circ \beta_s )\circ \xi (u)=
\alpha_s \circ (\beta_s \circ \xi(u))=
\alpha_s\circ (\psi(u)\circ \beta_t)=$$$$
(\alpha_s\circ \psi(u))\circ \beta_t=
(\phi(u)\circ \alpha_t)\circ \beta_t=
\phi(u)\circ (\alpha_t\circ \beta_t)\tsk$$

The unit transform $1_\phi: \phi\rightarrow \phi$
is defined with collection of   unit arrows
$1_{\phi_0(s)}:\phi_0(s)\rightarrow \phi_0(s)$.
It obviously  also meets the property of commuting diagrams.

So for arbitrary category $Y$ we have constructed the category
$Y^{(T)}$ which will be called an
^{=exponential  category}. It  defines  an  appointment of objects
for an ^{=exponential  superfunctor}.

Functors between the categories will be arrows  in category $\CAT$
and  will be also mapped by superfunctor.
For the functor $g: Y\doublerightarrow Y'$ we define a functor
between exponential
categories $g^{(T)}: Y^{(T)}\doublerightarrow (Y')^{(T)}$.
For each functor $\phi:T\doublerightarrow Y$
we appoint a new functor provided with changing of target space
 $\phi\circ g: T\doublerightarrow Y'$,
and for each natural transform $\alpha: \phi\rightarrow \psi$ we get
a new natural transform  $\alpha\times g: \phi\circ g\rightarrow \psi\circ g$.

We must check that for an identity functor
$\Identity_Y:Y\doublerightarrow Y$
we get again the identity functor over exponential category
$$(\Identity_Y)^{(T)}=\Identity_{(Y^T{())}}\kbl$$
and for a  composition of functors $g\circ k$ we get the
composition of functors
between exponential  categories
$$(g\circ k)^{(T)}= g^{(T)}\circ k^{(T)}\tsk$$

Such both superfunctors we have  defined even for
the category of graphs.
Now the associative composition
of arrows allows us to have truly joint pair of superfunctors
with counit arrows defined by collection of ^{=evaluation functors}
$$\ev_Y: Y^{(T)}\times T\doublerightarrow Y\tsk$$
Possibility to use natural transforms together with
 associative arrows composition
is essential.

For some functor $\phi: T\doublerightarrow Y$ and a  point  in source
category  $s\in T$ it appoints
the point in the target category $\phi(s)\in Y$, and  for a  natural
transform $\alpha: \phi\rightarrow \psi$
and an arrow in source category $u:s\rightarrow t$ it appoints
the composition of arrows
$$\phi(u)\circ \alpha_b = \alpha_a \circ \psi(u): \phi(s)\rightarrow
\psi(t)\tsk$$
First we need to check that such application maintains the composition of arrows.
Let we have another natural transform $\beta: \psi\rightarrow \xi$
and arrow
in the source category $\ell: t\rightarrow r$. Then

$$\matrix {\phi(s) &  & &   &  \cr
        \downarrow &\searrow &&  & \cr
        \psi(s)&\rightarrow &  \psi(t) &   &\cr
        \downarrow &    &\downarrow & \searrow && \cr
        \xi(s) & \rightarrow &  \xi(t)& \rightarrow& \xi(r)\cr}$$
\vskip\tarpas
and we need to check the equalities
$$(\alpha_s \circ \psi(u)) \circ (\beta_t \circ \xi(\ell))=
$$$$ \alpha_s \circ (\psi(u)\circ \beta_t)\circ \xi(\ell)=
$$$$ \alpha_s \circ (\beta_s \circ \xi(u))\circ \xi(\ell)=
$$$$(\alpha_s \circ \beta_s )\circ (\xi(u)\circ \xi(\ell))\tsk$$
\vskip\tarpas

For a transform with unit arrows $\alpha_s=1_{\phi(s)}$ and a unit arrow
in the source category
$1_s: a\rightarrow a $ we also get a unit arrow in the target category
$$ 1_{\phi(s)}\circ \phi(1_s)= 1_{\phi(s)}\tsk$$
This completes the checking that we indeed have got a functor
$Y^{(T)}\times T\doublerightarrow Y$.

We have projection of category of categories $\CAT$ to the category of
all sets $\SET$.
This is also an instance of superfunctor $\CAT\superrightarrow \SET $.
For each category $X$ we appoint its points set $X_0$, and
for a functor $f: X\doublerightarrow Y$ we have the appointment of points sets
$f: X_0\rightarrow Y_0$.
Obviously we have maintenance of composition  for  functors
and for the identity   functor $\Identity_X: X\doublerightarrow X$
it appoints the identity appointment  of points set
$\Identity_X: X\rightarrow X$. This projection will be called a ^{primary
=projection}.

The commuting diagrams from the category $\CAT$
rest commuting in the category of sets $\SET$.
Each joint pair of superfunctors in the category $\CAT$
$$\lan F,G\ran : \CAT \rightleftarrows \CAT $$
provides the joint pair of projected functors in the category $\SET$
$$\lan F_0,G_0\ran :  \SET \rightleftarrows \SET \tsk$$
The  study of unit and counit transforms
must be begun by investigation of their  projections.

 The  constructed Carte tensor product of categories  $X\times Y$
is projected to the
Carte tensor product of sets $X_0\times Y_0$, i. e. we have commuting
diagram of superfunctors

$$\matrix { \CAT \times \CAT & \mapright X\times Y & \CAT \cr
     \downarrow  & &\downarrow \cr
         \SET\times \SET & \maprightap X_0\times Y_0 & \SET \cr} $$
 \vskip \tarpas

For the  exponential functor $Y^{(T)}$ we additionally  apply  the
deformation. We change the set of graph transforms
$\phi: T\doublerightarrow Y$
by  the set of points  appointments $\phi_0: T_0\rightarrow Y_0$
and we get another
projection $\CAT \superrightarrow \SET$, which will be called a
^{secondary =projection}.

The  equality of two arrows $f,g: X\doublerightarrow Y$
in category $\CAT$ is defined
as equality for primary projections
$f_0,g_0: X_0\rightarrow Y_0$ in the category
$\SET$ and equality of arrows appointments
$$f_{x,x'}= g_{x,x'}: X(x;x')\rightarrow Y(f_0(x);f_0(x'))=
Y(g_0(x);g_0(x'))\tsk$$

For the joint pair of functors $X\times A$ and $Y^{(T)}$
in the category of all categories $\CAT$
we shall construct  unit and counit transforms.
The unit transform for joint pair of superfunctors
$$\Identity_{\CAT} \rightarrow FG$$
will be defined with the  collection of ^{=sections functors}
$$\lambda_X: X\doublerightarrow (X\times T)^{(T)}\tsk$$

It for a point $x\in X$ appoints the ^{=section}
$$\lambda_X(x): T\doublerightarrow X\times T$$
which for a point $s \in T$
appoints the couple $\lan x,s\ran \in X_0\times T_0$
and for an arrow in assistant category
$u\in T(s;t) $ appoints the arrow in the product of categories
$$\lan 1_x, u\ran \in X\times T\tsk$$


For an arrow $\theta\in X(x;y)$ it appoints the
natural transform between two sections
defined with the collection of arrows
$$\theta \times 1_s\in X\times T(\lan x, s\ran;\lan y,s\ran) \tsk$$

We can see that the composition of two arrows $\theta: x\rightarrow y$ and
$\rho: y\rightarrow z$ is mapped to the composition of natural transforms
between section functors
$$(\theta\circ \rho)\times 1_s= (\theta\times 1_s )\circ
(\rho\times 1_s)\tsk$$
and a unit arrows $1_x: x\rightarrow x$
will provide the identity transform between the same section
functor
$$1_x \times 1_s: \lambda_X(x)\rightarrow \lambda_X(x)\tsk$$
So we indeed have defined functors.

Such sections functors $\lambda_X: X\doublerightarrow (X\times T)^{(T)}$
defines natural transform between correspondent superfunctors.
For arbitrary  functor $f:X\doublerightarrow X'$ the
superfunctor appoints another  functor
$(f\times \Identity_T)^{(T)}: (X\times T)^{(T)}\doublerightarrow
(X'\times T)^{(T)}$ with commuting quadrat
\vskip\tarpas
$$\matrix{ X & \mapright f &X' \cr
          \mapdownk \lambda_X  & & \mapdownd \lambda_{X'} \cr
(X\times T)^{(T)} & \maprightap (f\times 1_T)^{(T)} & (X'\times T)^{(T)}
\cr} $$
\vskip \tarpas
At first we wish to  check that the primary projection provides
commuting quadrats in the category $\SET$. With secondary projection
we get ^{=sections appointments} in the category $\SET$
$$\lambda_{X_0}: X_0 \rightarrow (X_0\times  T_0)^{T_0} \kbl$$
therefore they will be arrows for natural transforms between
 superfunctors in the category $\SET$.

To get
 commuting diagram for the primary projection   we need
to check that the section
$\lambda_X(x)\in (X\times T)^{(T)}$
is mapped by functor $(f\times \Identity_T)^{(T)}$
to  another section
$\lambda_{X'}(f_0(x))\in (X'\times T)^{(T)}$.
This is not obvious  only for an  appointment of arrows.

For arbitrary arrow $u\in T(s;t)$ the first section
$\lambda_X(x)$ appoints an arrow $$\lan 1_x, u\ran\in
X\times T(\lan x,s\ran;\lan x,t\ran)$$
and the functor $(f\times \Identity_T)^{(T)}$
appoints another section $\lambda_{X'}(f_0(x))$, which for arbitrary arrow
$u\in T$ provides the arrow
$$\lan 1_{f_0(x)}, u\ran \in X'\times T(\lan f_0(x),s\ran;
\lan f_0(x),t\ran)\tsk$$
This value will be the same for the section get in category $X'$
with the changed point $f_0(x)\in X'_0$.

It rests to check commuting diagram for arrows appointments.
For an arrow $\theta\in X(x;y)$ we appoint a natural
transform between section
$$\lambda_X(x)\rightarrow \lambda_X(y)$$
defined with the collection of arrows
$$\theta\times 1_s\in X\times T(\lan x,a\ran;  \lan y,a\ran) \uparrow s\in T$$

The functor $(f\times 1_T)^{(T)}: (X\times T)^{(T)}\doublerightarrow
 (X'\times T)^{(T)}$
appoints the natural transform   defined with a
new collection of arrows
$$\lan f(\theta), 1_s\ran \in X'\times T( \lan f_0(x),s\ran;
\lan f_0(y),s\ran)\uparrow s\in T_0
\tsk$$
This indeed coincides with the natural transform appointed
by the  functor
$\lambda_{X'}: X'\doublerightarrow (X'\times T)^{(T)}$
to an arrow
$f(\theta)\in X'(f_0(x);f_0(y))$.

The counit transform
$$GF\rightarrow \Identity _{\CAT} $$
will be defined by collection of evaluation functors
$$\ev_Y: Y^{(T)}\times T\doublerightarrow Y\tsk$$
This transform is natural.
We need to check 
commuting diagrams for arbitrary functor
$g: Y\doublerightarrow Y'$
\vskip\tarpas
$$\matrix{ Y^{(T)}\times T& \mapright {g^{(T)}\times 1_T} &
(Y')^{(T)}\times T\cr
           \mapdownk \ev_Y &               &\mapdownd \ev_{Y'} \cr
           Y & \maprightap g   & Y' \cr } $$
\vskip \tarpas

Their secondary projection will be the evaluation appointment for functional
set in the category $\SET$
$$\ev_{Y_0}: (Y_0)^{T_0}\times T_0 \rightarrow  Y_0 \kbl$$
therefore in category $\SET$ we get  arrows  for  natural transform.

We can see that the primary  projection also defines natural transform
between superfunctors in the category $\SET$.

The primary projection of evaluation functor
$\ev_Y: Y^{(T)}\times T\doublerightarrow Y$
for a functor $\phi: T\doublerightarrow Y$ and a point $s\in T_0$ appoints
the value $\phi_0(s)\in Y_0$ of points appointment
$\phi_0: T_0\rightarrow Y_0$, i. e. depends only from second projection of
exponential category $Y^{(T)}$.

It rests to check commuting diagram for the arrows appointment.
Let we have a natural transform $\alpha: \phi\rightarrow \psi$
between two functors $\phi,\psi\in Y^{(T)}$ defined by collection of
arrows $\alpha_s\in Y(\phi_0(s);\psi_0(s))\uparrow s\in T$
and an arrow in an assistant category $u\in T(s;t)$. Then functor
$g^{(T)}\times \Identity_T: Y^{(T)}\times T\doublerightarrow
(Y')^{(T)}\times T$
appoints  the new natural transform between new functors with
changed target space
$$\alpha\times g: \phi\circ g \rightarrow \psi\circ g$$
 defined
by collection of arrows $g(\alpha_s)\in  Y'( g_0(\phi_0(s));g_0\psi_0(s)))\uparrow
 s\in T$ and the same arrow in assistant category $u\in T(s;t)$.

Otherwise the evaluation functor $\ev_{Y'}$ will appoint the diagonal
arrow
$$g(\alpha_s)\circ \psi(u)\in Y'(g_0(\phi_0(s));g_0(\psi_0(t)))$$
the same as  the image of arrow $\alpha_s\circ \psi(u)\in
Y(\phi_0(s);\psi_0(t))$
$$g(\alpha_s\circ h)= g(\alpha)\circ g(u)\tsk$$

For the truly joint pair of  superfunctors $X\times T$ and $Y^T$
we must check both triangular equalities for unit and counit transforms.
It can be seen by earlier proved propositions for graphs transports.

We can  apply the proposition about bijective name mapping between
sets of functors
$$\CAT (X\times T; Y)=\rightarrow \CAT(X;Y^{(T)})\tsk$$
The unit arrows $1_x\in X(x;x)$ are maintained by any functor, and they
are neutral for
arrows composition.
The functor $f: X\times T\doublerightarrow Y$ is decomposable for the
arrows composition in target category $Y$, as we have equality in product
category
$$\lan \alpha, 1_s\ran \circ \lan 1_b\circ u\ran =\lan
 \alpha\circ  1_b, 1_s\circ u \ran= \lan \alpha, u\ran\uparrow \alpha\in X(a;b),
 u\in  T(s;t)\tsk$$
  So we get injective name mapping
to the set of functors corestricted in the exponential space of natural
transforms. The realization mapping is also injective over such set
of functors. Therefore both name mapping and realization mapping
are bijective.

The bijective name mapping provides both triangular equalities.
The first triangular equality is  the property for realization  mapping
to reverse the name of identity functor
$$\Identity_{X\otimes T}: X\otimes T\doublerightarrow X\otimes T \tsk$$
The second triangular equality is the property for name mapping  to reverse
the realization of identity functor
$$\Identity_{Y^T}: Y^T\doublerightarrow Y^T \tsk$$
So we have proved already these properties. Nevertheless
we shall check these triangular equalities once more without applying
the proposition on bijective name mapping in category of graphs.
However we shall only repeat the earlier proving for this special case.

The first triangular equality is for the unit transform ended with the
adjoint superfunctor
and composed with the counit transform  begun with the adjoint superfunctor
$$(i\times F)\circ (F\times e) = 1_F\tsk$$
The first natural transform is defined by collection of sections functors
$$\lambda_X\times \Identity_T: X\times T\doublerightarrow
(X\times T)^{(T)}\times T \kbl$$
the second natural transform is defined by collection of evaluation functors
$$\ev_{X\times T}: (X\times T)^{(T)}\times T\doublerightarrow X\times T\tsk$$

The triangular  equality in the category
$\SET$ we have for the secondary projection. It is also valid for the primary projection, as evaluation functors
depends on secondary projection only.

So it rests to check the triangular equality only for arrows appointments.

For a couple of arrows
$\lan \theta,u\ran\in X\times T(\lan x,s\ran;\lan y,t\ran) $
the sections  functor appoints the natural transform between two sections
$ \lambda_X(x),\lambda_X(y)\in Y^{(T)}$
defined with collection of couples compounded by arrows
$$\lan \theta, 1_s\ran\in  X\times T(\lan x,s\ran;\lan y,s\ran)$$
and the identity functor $\Identity_T: T\doublerightarrow T$
appoints the same arrow in assistant
category $u\in T$.

Further the evaluation functor  in the category
$X\times T$  appoints the diagonal arrows
$$\lan \theta, 1_s\ran \circ \lambda_X(y)(u)=
\lan \theta,1_s\ran\circ \lan 1_y,u\ran= \lan \theta,  u\ran \in
 X\times T(\lan x,s\ran;\lan y,t\ran)\tsk$$
So we have got the same couple of arrows.

The second triangular equality is for the unit arrow begun
with the coadjoint superfunctor $G$
and composed with the counit arrow  ended with the coadjoint superfunctor $G$
$$(G\times i)\circ (e\times G)=1_G\tsk$$
This composition must be identity transform defined by collection of
the identity
functors  over  exponential categories $Y^{(T)}$.

The first natural transform
is defined by collection of  sections functors
 $$\lambda_{Y^{(T)}}: Y^{(T)}\doublerightarrow (Y^{(T)}\times T)^{(T)}$$
and the second natural transform is defined with  collection of
changing target space by evaluation functor
$$(\ev_Y)^{(T)}: (Y^{(T)}\times T)^{(T)}\doublerightarrow Y^{(T)} \tsk$$
For the secondary projection we have the
triangular equality in the category $\SET$
We need to check such triangular equality also for the primary
projection.

For a functor $\phi: T\doublerightarrow Y$ we must check that for an arrow
$u'\in T(s';t')$ finally we appoint the value
$\phi(u')\in Y(\phi_0(s');\phi_0(t'))$ of the same functor $\phi$.

The first sections functor will appoint the section
$\lambda_{Y^{(T)}}(\phi):T\doublerightarrow Y^T\times T$
which for a point $s'\in T_0$ will appoint the couple
of points $\lan \phi, s'\ran \in Y^{(T)}
\times T $ and  for an arrow $u'\in T(s';t') $ it appoints the couple
of arrows
$$\lan \phi,u'\ran \in  Y^{(T)}\times T(\lan \phi,s'\ran;\lan \phi,t'\ran)
\tsk$$
Changing the target space with evaluation functor
$\ev_Y: Y^T\times T  \doublerightarrow Y$ provides the diagonal arrow
$$1_{\phi_0(s')}\circ \phi(u')=\phi(u')  \in Y(\phi_0(s');\phi_0(t'))\tsk$$

It rests to check identity appointment
for the  composition of arrows appointments.
For the natural transform $\alpha:\phi\rightarrow \psi$ between functors
$\phi:T\doublerightarrow Y$ and $\psi: T\doublerightarrow Y$
the first sections functor
will appoint a natural transform between two sections
$$\lambda_{Y^T} (\phi)\rightarrow \lambda_{Y^T} (\psi)$$
defined with the collection of arrows
$$\lan \alpha, 1_{s'}\ran: \lan \phi,s'\ran \rightarrow
\lan \psi, s' \ran \uparrow s'\in T_0$$
which are natural transforms between functors $T\doublerightarrow
Y^{(T)}\times T$,
 defined with collections of arrows
$\lan \alpha_s, 1_{s'}\ran \in  Y\times T(\lan \phi_0(s),s'\ran;
\lan \psi_0(s),s'\ran) $.
The changing target space with the evaluation functor
$\ev_Y: Y^{(T)}\times T\doublerightarrow Y$
for every couple $\lan \alpha,  1_{s'}\ran \in Y^{(T)}\times T(\lan \phi,s' \ran;
\lan \psi,s'\ran )$ will appoint the diagonal arrow
$$\alpha_{s'}\circ 1_{s'}= \alpha_{s'} \in T(\phi_0(s');\psi_0(s'))\tsk$$
So we have shown completely the second triangular equality.

The bijective realization mapping
$$f: X\times T\mapright g Y^{(T)}\times T \mapright \ev_Y  Y$$
can be interpreted as arrow of unit transform
$\lambda_X: X\doublerightarrow (X\times T)^{(T)}$
 to be initial in ^{=comma category }  $$(X\downarrow G)$$
for exponential superfunctor of natural transforms
$Y^G= Y^{(T)}$. The functors $X\doublerightarrow Y^G$  are taken as points
and commuting functors between target spaces $h: Y\doublerightarrow Y$
are taken as arrows of comma category $(X\downarrow G)$. The bijectivity of
realization mapping provides that for each functor $m:X\doublerightarrow Y^G$
unanimously exists an arrow $n:F(X)\doublerightarrow Y$ which realization
coincides with taken arrow, i. e.
$$\lambda_X\circ n^G= m \tsk$$

The initial arrow is unique up the unique isomorphism, therefore
we can construct unique isomorphism between
two possible exponential functors. However it is hard imagine what can
be another exponential functor aside the exponential functor of natural
transforms $Y^{(T)}$.   This will be useful when we shall apply the notion
of equalizer to define the exponential space of natural transforms $Y^{(T)}$.
Equalizer is also defined unanimously  up unanimously defined isomorphism.

Interesting  to apply such constructions even in cases when exponential
space of natural transforms doesn't maintain composition of arrows, i. e.
isn't superfunctor. 
\vskip\tarpas
We present once more another closed monoidal category of Banach spaces
$\Ban$. Such spaces were introduced by \baf S. Banach 1922*.
Banach space $X$ can be presented as complete metric  space with
linear structure.  In Banach space  $X$
we have additive Abel group with addition of vectors
$$+: X\times X\rightarrow X $$
and additive homothety by scalar $r\in \VR$
$$r: X\rightarrow X \tsk$$
Such linear structure we can understood as a convergence for finite
sequences. Additionally we introduce a metric with norm
$$X(x;y)= \Vert y-x\Vert \in \VR_+ \tsk$$
We demand that taken vector space $X$ would be complete for Cauchy
sequences of such metric.
The morphism between two Banach spaces will be taken bounded linear
 mappings
$u: X\rightarrow X$ with  bounded norm
$$\Vert u\Vert= \sup_{ \Vert x \Vert\mzl 1} \Vert u(x)\Vert \mz +\infty\tsk$$

The ^{algebraic tensor =product} is defined as an initial object
in the  bilinear
mappings $U\times V\rightarrow W$ with commuting triangular diagram
defined by linear mappings of target spaces $W\rightarrow W'$.
Therefore for existing of tensor product  $U\otimes V$
with bilinear mapping
 $U\times V\rightarrow U\otimes V$  and arbitrary other bilinear mapping
 $U\times V\rightarrow W$ we have exactly one linear mapping
  $U\otimes U\rightarrow W$ providing commuting diagram
$$\matrix { U\times V & \rightarrow & U\otimes V \cr
          \downarrow & \swarrow & \cr
          W &        &  \cr } $$
\vskip\tarpas
Constructing of such algebraic tensor product of linear spaces can be
seen in  \baf N. Bourbaki Alg\`ebre, chp. 3. Alg\`ebre multilineaire.*

The ^{projective tensor =product} of Banach spaces $U$ is defined as
completion of
metric space on algebraic tensor product $U\otimes V$ with
projective product of norms
$$p_1\sqprod p_2(u)= \inf\lbrace \sum_i p_1(x_i)p_2(y_i) : u= \sum_i
x_i\otimes y_i\rbrace \tsk$$
cl. Topological tensor products in
\baf  H. Schaefer 1966* part III. Linear mappings  \S 6.
For arbitrary Banach space $Z$ we have isometrical
bijection between the space of bilinear mappings
$f: X\times Y \rightarrow Z$ with norm
$$\Vert f\Vert= \sup_{\Vert x\Vert\mzl1,\Vert y\Vert\mzl1} \Vert f(x,y)\Vert$$
and correspondent linear mappings  $u: X\sqprod Y\rightarrow Z$ with
norm $$\Vert u\Vert= \sup_{\Vert x\Vert\mzl1,\Vert y\Vert\mzl1}
\Vert u(x\otimes y)\Vert \tsk$$
The correspondent linear mapping is produced as continuous extension of
linear mapping defined by bilinear mapping over algebraic tensor product.

The points of projective tensor product $ u\in U\sqprod V$
are expressed as absolutely convergent sum
$$u= \sum_{i\dgl 1} \lambda_i x_i\otimes y_i$$
with $\sum_{i\dgl 1} |\lambda_i| \mz +\infty$ and
$x_i\in U$, $y_i\in V$ are sequences converging to zero point.
This characterization is proposed in  \baf A. Pietsch 1963*.

We shall check again that the category of Banach spaces $\Ban$ with
projective tensor product $U\sqprod V$ is closed monoidal category.

For arbitrary assistant Banach space $A$ we define adjoint functor
which for the Banach space $U$ appoints a new Banach space $U\sqprod A$
and for bounded linear mapping $u: U\rightarrow U'$ it appoints a new
bounded linear mapping
$$u\times 1_A: U\sqprod A\rightarrow U'\sqprod A\tsk$$

The coadjoint functor for the arbitrary Banach space $V$ appoints
a new Banach space $V^A$ compounded of all bounded linear mappings
$\phi: A\rightarrow V$. For bounded  linear  mapping $v: V\rightarrow V'$
it appoints changing of target space  $g_*: V^A\rightarrow (V')^A$
which for a mapping $\phi\in V^A$ appoints the composed  mapping
 $$v\circ \phi: A\rightarrow (V')^A\tsk$$
 
 The unit transform for joint pair of  functors
 will be defined by collection of sections mappings
 $$\lambda_U: U\rightarrow (U\sqprod A)^A\tsk$$
We have section $\lambda_U(x):A\rightarrow U\sqprod A$ which for the point
$s\in T$ appoints a tensor  $x\otimes a\in U\sqprod A$ with  norm
$$\Vert x\otimes a\Vert= \Vert x\Vert\cdot \Vert a\Vert\kbl$$
so we get section's norm
$$\Vert \lambda_U(x) \Vert= \sup_{\Vert a\Vert\mzl1}
\Vert x\otimes a\Vert=\Vert x\Vert\kbl$$
and the norm of sections mapping
$$\Vert \lambda_U\Vert= \sup_{\Vert x\Vert\mzl1} \Vert x\Vert= 1\tsk$$

The  counit transform will be defined
 by collection of evaluation mappings
 $$\ev_V: V^A\sqprod A\rightarrow V\tsk$$
At first it is defined as a bilinear continuous mapping
$$\ev_V(\lan \phi,s\ran)= \phi(s)$$ with inequality for norm
$$\Vert \phi(s)\Vert \mzl\Vert \Phi u \Vert\cdot \Vert a\Vert\tsk$$
Then we take  its continuous extension
over projective tensor product.

Both triangular equalities for truly joint pair of functors
$$\lan F, G\ran: \Ban \rightleftarrows \Ban $$
is provided by such equalities in larger category $\Set$, or
smaller category of convergence spaces with continuous mappings.

Instead we shall show with some  difficulties
that we have natural bijection between sets of bounded linear mappings
$$\Ban( U\sqprod A; V)=\rightarrow \Ban (U;V^A)\tsk$$

For a bounded linear mapping $\Phi: U\sqprod A\rightarrow V$ we get
a continuous bilinear mapping $U\times U\rightarrow V$, therefore
it will be partially continuous, so we get continuous linear
mapping $\Phi_1: U\rightarrow V^T$. Otherwise for arbitrary
continuous mapping  $\Psi: U\rightarrow V^T$ we get partially continuous
bilinear mapping $U\times A\rightarrow V$, which for  Banach space
will be continuous, so it  has an extension over the whole projective
tensor product $\Phi(x\otimes y)= \Psi(x)_y $.

In  the category $\Ban$ we can take another tensor product.
For two Banach space $U$ and $V$ we appoint ^{biequicontinuous
tensor =product}
$U\bar {\sqprod}  V$.
On algebraic tensor product $U\otimes V$ we take a norm of uniform
convergence  over tensor product of equicontinuous sets.
For tensor $u= \sum_{i\dgl 1} x_i\otimes y_i $ we take
a norm  defined with continuous forms $f\in U'$ and $g\in V'$
$$[u]= \sup_{\Vert f\Vert \mzl 1, \Vert g\Vert\mzl 1}
\sum_i \lan x_i,f\ran\cdot \lan y_i,g\ran \tsk$$
So we get a smaller norm
$$[u]\mzl \sum_{i\dgl 1} p_i(x_i)\cdot p_2(y_i)\kbl$$
therefore $[u]\mzl p_1 \sqprod p_2(u)$ and
we have got a bounded imbedding
$$U\sqprod V\subset U\bar{\sqprod} V\tsk$$
In \baf H. Schaefer 1966* part IV. Duality  \S9.2 we can see
the dual space for biequicontinuous tensor product $X\barsqprod Y$.
It  coincides with the space of integrable mappings
$f: X\barsqprod Y \rightarrow \VR$
defined with Radon measure over weakly compact space
$\mu\uparrow S\times T$ with
$S= \lbrace x': \Vert x'\Vert\mzl 1\rbrace\subset X'$  and
$T= \lbrace y': \Vert y'\Vert\mzl 1\rbrace\subset Y'$.
$$f(u)= \int \mu \dfc \lan x', y'\ran \cdot \lan u, x'\otimes y'\ran \tsk$$

For  Banach space $Z$ the continuous linear mappings
$f: X\barsqprod Y \rightarrow Z$ is defined by bounded vector measure
$\mu\uparrow S\times T$  with the equalities for scalar forms
$$\lan f(u),z' \ran= \int\lan  \mu, z'\ran \dfc \lan x',y'\ran \cdot
\lan u , x'\otimes y'\ran \tsk$$
We demand that scalar measures would have uniformly bounded variations
$$\sup_{\Vert z'\Vert\mzl 1} \Vert \lan \mu, z' \ran \Vert\mzl C\tsk$$

Once again we want to get a joint pair of functors. We take adjoint
functor  defined
by new tensor product
$U\bar {\sqprod} V$. The coadjoint functor  would be defined with
the same exponential space $V^A$ compounded of continuous
linear mappings with the norm of
uniform convergence over the unit ball in
the space $A$
$$\Vert u\Vert= \sup_{\Vert a\Vert\mzl 1} \Vert u(s)\Vert \tsk$$

However we must take a smaller category to get again truly
joint pair of
 functors. Difficulties arises with evaluation mapping.
It must be continuous for weaker topology of biequicontinuous tensor
product
$$\ev_Y:Y^A\bar {\sqprod} T\rightarrow Y\tsk$$
This problem is solved taking integrable linear mappings.

The integrable mappings between two Banach spaces $u:U\rightarrow V$
is defined by integral of bounded vector measure  $\mu \dfc x' $
over weakly compact set
in dual source space  $U'$
$$B^\circ= \lbrace x'\in U' : \lan  x,x' \ran\mzl 1 \uparrow \Vert x\Vert\mzl 1
\rbrace\tsk$$
We shall denote
$$u= \int \mu \dfc x' \cdot x'$$
and its values are unanimously   defined
by scalar integrals             
$$\lan u(s), y'\ran = \int \lan  \mu,y'\ran  \dfc x' \cdot \lan a, x'\ran
\in \VR\uparrow y'\in Y'\tsk$$
For bounded vector measure we shall have an inequality
$$\sup_{\vert y'\vert\mzl 1}  \lan u(s), y'\ran \mzl
\sup_{\Vert y'\Vert\mzl 1}  \int |\lan \mu , y'\ran | \dfc x'\cdot
\Vert a \Vert \mzl  C\cdot \Vert a\Vert\tsk$$

We shall define a smaller category of Banach spaces $\SBan\subset \Ban $
leaving as arrows  only the integrable linear mappings.
First we must check is the identity mapping integrable.
For this we need construct  a weak base  in Banach spaces. \baf
 J. Schauder  1927*  for some Banach spaces  constructed topological base
 $x_i\in X\uparrow i\in I$  with dual collection of linear forms
 $f_j\in X'\uparrow j\in X'$ permitting the orthogonal
 relations
 $$\lan x_i, f_j\ran= \delta_{i,j}\uparrow i,j\in I $$
and  providing sums unconditionally converging in initial
 topology of Banach space
 $$\sum_{i\in I} x_i f_i(x) = x \tsk$$
 \baf S. Karlin 1948*
has shown that there isn't any such base even in a space of continuous
scalar  functions
over compact interval $\VC\uparrow [0,1]$. However for weak
topology such bases exist always  for every Banach space $X$.
More exactly
we have continuous imbeddings
$$\ell^1 \subset X\subset \ell^\infty\kbl \ell^\infty\supset X'\supset
\ell^1 $$
for some collection of vectors $x_i\in E\uparrow i\in I$ and forms
$f_i\in E'\uparrow i\in I $ with orthogonality condition
$$\lan x_i,f_j \ran= \delta_{i,j}\kbl \Vert x_i\Vert=1 \kbl \Vert f_j\Vert=1
\tsk $$

\Proposition
In Banach space $X$ we  can find a weak topological basis
$x_i \in B$, $\Vert x_i\Vert=1$  with dual
collection  of continuous forms $f_j\in X'$
$$\lan x_i, f_j\ran= \delta_{i,j} \tsk$$
\Proof:
In \baf H. Schaefer 1966* part II. Locally convex spaces \S 4.2
Corollary 1 of theorem we can see construction of such collection of forms
$f_j\in X'$ for arbitrary finite collection of independent vectors
$x_i\in X$.
We extend this construction by infinite induction for arbitrary Banach
space,

Let we have a collections  of independent vectors
$x_i\in X$, $\Vert x\Vert=1$  and
continuous forms $f_j\in X'$, $\Vert f_j\Vert=1$
with orthogonality relation
 $$\lan x_i,f_j\ran=\delta_{i,j} \uparrow i,j\in I \tsk$$
Let these vectors $x_i\in X$ generate  closed linear subspace
$E \subset X$. By Hahn 1928 and Banach 1929 theorem generated closed linear
space is characterized by property for arbitrary continuous form
$f\in X'$ to vanish if it vanishes over each basic vector
$$f(x_i)= 0 \uparrow i\in I\duoda f(E)=0\tsk$$

If $E\not= X$, we can find
a form vanishing for basic vectors $f(x_i)= 0\uparrow i\in I$ and having
not zero  value $f(x)\not =0$
   over some vector $\Vert x\Vert =1$.
We want find such point in intersection of zero spaces of all
basic forms
$$x\in \Cap_{j\in I} f_j\inv (0)\tsk$$

For arbitrary summable series of scalars $\sum_j|\alpha_j |\mz +\infty$
we get a continuous form again
$$\sum_j \alpha_j f_j \in X'\tsk$$
and for arbitrary $x\in X$ we get  a bounded series
$$\sup_j f_j(x)\mz +\infty\tsk$$
So we get continuous imbeddings
$\ell^1\subset X'\subset \ell^\infty$.
The similar dual imbeddings we have for the space $X$ itself
$\ell^\infty\supset X \supset \ell^1$
as for the summable series of scalar $\beta_j\uparrow j\in I$
we get a point $x= \sum_j \beta_j x_j $, and for each point $x\in X$
we appoint a bounded sequence of scalars $f_i(x)\uparrow i\in I$.
We have equalities of dual mappings
$$\lan x,i(\alpha_i)\ran_{X\times X'}= \lan (f_i(x) ),(\alpha_i)
\ran_{\ell^\infty \times \ell^1}\kbl$$
$$\lan \sum\beta_j x_i , f\ran_{X\times X'} = \lan (\beta_j), (f(x_j))
\ran_{\ell^1\times \ell^\infty} \tsk$$

By \baf H. Schaefer 1966*  Part IV. Duality \S 2.3
for dual mappings we have equality of polars
$$u(s)^\circ = (u')\inv (A^\bullet)\tsk$$
So for the image of the whole space $u(\ell^1)\subset X$ we get
a polar
$$(u')\inv (0)\subset X'\kbl$$
i. e. for all basic mappings $f_i$ we have  $f_i(x) =0$.

Otherwise for some summable series
$$x=\sum_i \beta_i x_i \in X$$
with $f(x)\not =0 $ we can correct this point
$$x'= x-\sum_j \beta_j x_i \in X$$ to get
$f(x')=f(x)\not=0$ and $f_i(x')=0$ for all $i\in I$.

We take such $x\in X$ with unit norm
$\Vert x\Vert=1$ as next point in the collection of basic points
$(x_i\uparrow i\in I)$ and define next basic form
with $f(x)=1$. So we have got  for all $i\in I$
$$f_i(x)= 0\kbl f(x_i)=0\kbl f(x)=1 \tsk$$

After such construction we can apply infinite  induction
to provide a maximal collection of basic points $x_i\in X$ and dual basic
forms
$f_i\in X'$. For it we shall have injective dual linear mappings
$$\ell^1\subset X\subset \ell^\infty \kbl
\ell^\infty \supset X' \supset \ell^1 \tsk$$
\irodymopabaiga

Weak base in Banach space $x_i\in X$ with dual collection of basic
forms $f_i\in X'$
provides integrable presentation of identity mapping
$\Identity_X: X\rightarrow X$
$$x =\sum_{i\in I} x_i \otimes f_i (x) $$
with vector measure
$$\lan \mu,y'\ran \dfc x'= \sum_{i\in I} \lan x_i,y'\ran  f_i  \tsk$$

Without such representation we could work only with
semicategory of integrable mappings. Such situation will be inevitable
 with the
semicategory of compact linear mappings.

The composition of two integrable linear mappings rests integrable.
If we have integrals of vector measures
$$\lan u(x), y'\ran = \int \lan \mu, y'\ran  \dfc x'\cdot \lan x,x'\ran \kbl
\lan v(y), z'\ran = \int \lan \nu, z'\ran  \dfc y'\cdot \lan y,y'\ran \kbl$$
then
$$\lan v(u(x)), z'\ran =\int \lan \nu,z'\ran \cdot \lan u(x),y'\ran
=
 \int \lan \nu, z'\ran \dfc y'\cdot \int \lan \mu , y'\ran \dfc x'\cdot
\lan x,x'\ran \tsk$$
So the composition is get by bounded vector measure
$$\lan \kappa, z'\ran = \int \lan \nu,z'\ran \dfc y' \cdot \lan \mu,y'\ran
\tsk$$

We have get a category $\SBan$ of integrable linear
mappings between Banach
spaces.

Exponential space $V^A$ will be compound by all integrable linear mappings
$u: A\rightarrow V$  with the same norm of uniform convergence over
unit ball in source space
$$\Vert u\Vert= \sup_{\Vert a\Vert \mzl 1} \Vert u(s)\Vert \tsk$$

The unit transform for joint pair of functors
will be defined by collection of sections mappings
$$\lambda_U: U\rightarrow   (U\bar{\sqprod} A)^A \tsk$$
For a point $u\in U$ it appoints the section
$\lambda_U(u): A\rightarrow U\bar {\sqprod} A$ with values
$$\lambda_U(u)_s= u\otimes a \tsk$$
Such section will have summable expression get from weak base in assistant
Banach space  $T$
$$u\otimes a= u\otimes (\sum_{i\in I} a_i  g_i(s))\tsk$$

The integral expression of sections mapping needs also weak base in
Banach space $U$
$$\lambda_U(u)= (\sum_{j\in J} u_j f_j(u))\otimes ( \sum_i
a_i\otimes g_i)\tsk$$

The counit transform  will be defined by collection of
evaluation mappings
$$\ev_V: V^A\bar{\sqprod} A\rightarrow V\tsk$$
It will be integrable linear mapping for integrable linear mappings
$\phi: A\rightarrow V$.
Let we have integrable expression
$$\phi(s)= \int \mu \dfc x' \cdot \lan a, x'\ran \in Y\tsk$$
Then evaluation mapping will be continuous over biequicontinuous
tensor product. For weakly continuous function $\phi$ its values can be checked
by Dirac measures. So  we get inequality

$$\phi(s)\mzl \sup_{\Vert \nu=1} \int \nu\dfc x'\cdot \phi(s)$$
with upper boundary is taken over all Radon measures on the ball in assistant
space $T$
$$\lbrace s\in T: \Vert a\Vert\mzl 1\rbrace $$
with weakly topology.
Also the polar of
unit ball $B\subset V^T$ will be compound
of bounded Radon measures $\nu\dfc x' $ over the
 ball in assistant space
$$\lbrace s\in T: \Vert a\Vert \mzl 1\rbrace \tsk$$
So we get an estimate
$$|\phi(s)|\mzl \sup_{\Vert \nu \Vert\mzl 1} |\int \nu\dfc a \cdot \phi(s)|
= $$$$\sup_{\Vert \nu\Vert\mzl 1, \Vert x'\Vert \mzl 1} |\int \nu\dfc a\cdot
\phi(s)|\cdot |\lan a,x'\ran|= [\phi\barsqprod a]\tsk$$

Both triangular equalities are the same as in larger category $\Ban$.
So we get truly joint functors $X\barsqprod A$ and $Y^T$ in  the category
$\SBan$ and  a natural bijections between sets of integrable linear mappings
$$\SBan (X\barsqprod A; Y)=\rightarrow \SBan (X; Y^A) \tsk$$
This can be deducted also from description of continuous linear mappings over
biequicontinuous tensor product in \baf H. Schaefer 1966* part IV. Duality
\S 9.2.
Continuous linear mappings over biequicontinuous tensor product of
Banach spaces $f: X\barsqprod T\rightarrow Y$ coincide  with integrable linear
mappings  get with Radon measures over polars of unit balls
$B=B_1(0)\subset X$ and $D= B_1(0)\subset A$
$$ f(u)= \int _{B^\circ \times D^\circ } \mu \dfc (x',s')\cdot u(x',s')\tsk$$
This can be expressed as integrable linear mappings  to the
 space $Y^A$
$$X\rightarrow Y^A \tsk$$
 We need only to apply integration of double integral
$$\int_{B^\circ \times D^\circ} \mu \dfc (x',s')\cdot u(x',s')=
\int_{B ^\circ} \nu\dfc x' \cdot \int_{D^\circ} \mu(x', \dfc  s')
\cdot u(x',s') \tsk$$
\vskip\tarpas
We can show that the biequicontinuous tensor product is a ^{=relator} for
the projective tensor product, i. e. we have bounded linear mapping
$$(X\barsqprod Y)\sqprod (Z\barsqprod W) \subset  (X\sqprod Y)\barsqprod
(Y \sqprod W)\tsk$$
It is enough to show continuity of correspondent bilinear mapping
$$(X\barsqprod Y)\times (Z\barsqprod W) \rightarrow  (X\sqprod Y)\barsqprod
( Y\barsqprod W) \tsk$$
This bilinear mapping is constructed by pairs of projections
$$p_1: X\barsqprod Y\rightarrow X\kbl q_1:Z\barsqprod W\rightarrow Z$$
and
$$p_2: X\barsqprod Y\rightarrow Y\kbl q_2: Z\barsqprod W\rightarrow W \tsk$$
Finally we get two continuous bilinear mappings
$$p_1\sqprod q_1: (X\barsqprod Y)\times (Z\barsqprod W) \rightarrow
 (X\sqprod Z) $$
 and
 $$p_2\sqprod q_2: (X\barsqprod Y)\times (Z\barsqprod W) \rightarrow
 (Y\sqprod W)\tsk$$
So we get also continuous biequicontinuous product
$$(p_1\sqprod q_1)\barsqprod (p_2\sqprod  q_2):
(X\barsqprod Y)\times (Z\barsqprod W) \rightarrow
 (X\sqprod Z) \barsqprod (Y\sqprod W)\tsk$$


\vskip\tarpas
Let in  arbitrary monoidal closed category $\VV$
with tensor product
$$r\otimes s\in \VV\uparrow r\in \VV, s \in \VV\tsk$$
we have another tensor product $r\sqprod s$ with a  property
$$  (r\sqprod r')\otimes
(s\sqprod s') \rightarrow (r\otimes s)\sqprod (r'\otimes s')
$$
and the same neutral object
$$*\sqprod r= r=r\sqprod *\tsk$$

We demand that such arrows would define natural transform
between two functors.

It will be called ^{=relator} to the previous tensor product.
Similar notion perhaps we can see in \baf R. Backhouse, P. Hoogendijk 2000*.
As a consequence we get an arrow
$$r\otimes s= (r\sqprod *)\otimes (s\sqprod *)\rightarrow (r\sqprod s)\otimes
(*\sqprod *)= r\sqprod s\tsk$$
They also define a natural transform between two functor, in this case
we have natural transform between two tensor products.

% Uýbaigiau clattice/closed.tex

